Modular Answer Set Programming as a Formal Specification Language

In this paper, we study the problem of formal verification for Answer Set Programming (ASP), namely, obtaining a formal proof showing that the answer sets of a given (non-ground) logic program P correctly correspond to the solutions to the problem encoded by P, regardless of the problem instance. To this aim, we use a formal specification language based on ASP modules, so that each module can be proved to capture some informal aspect of the problem in an isolated way. This specification language relies on a novel definition of (possibly nested, first order) program modules that may incorporate local hidden atoms at different levels. Then, verifying the logic program P amounts to prove some kind of equivalence between P and its modular specification. Under consideration for acceptance in TPLP.

==> approach.tex <==
%!TEX root = verification-modular-show.tex
\section{Nested modular programs}\label{sec:modlog}

\red
In the methodology presented here,  we propose the use of \emph{modular logic programs} as \emph{formal specifications}.
%
We depart from the work on modular logic programs by~\citeN{har16}, where each ``module'' of the modular program is a FO formula, whose semantics is captured by the SM operator.
%
This choice is motivated by two factors:
\begin{itemize}[noitemsep]
\item The first-order nature of Harrison and Lierler formalism,
which allows us to argue about the meaning of each module without grounding:
%
to use logic programs as a specification language, 
it is essential that the meaning of its parts can be assessed independently of any particular instance of the problem.
\item The SM operator -- a technical tool for capturing semantics of logic programs -- has been well studied in the literature and possesses a manifold of technical results (including  theorems on splitting or constraints, for instance) are readily available.
\end{itemize}
%
To adapt this modular approach to the needs of our goal,
we extend it  in two ways:
(i)~handling auxiliary predicates inside modules
% through a formal semantics for the directive {\tt \#show}
and (ii) introducing nested modules.


% We proceed to define now our extension of \cite{har16} that incorporates
% public predicates and nested modules.
%
A \emph{\definition} $\cM$ is a pair \mbox{$(\vec{p}:F)$}, where $\vec{p}$ is a tuple of intensional predicate symbols and $F$ is a \mbox{FO formula}.
%
Its  semantics  is captured by the formula $\Phi(M) \eqdef \SM_\vec{p}[F]$.
%
When $\vec{p}$ is empty, we write~$F$ in place of \definition \mbox{$(\vec{p}:F)$} --- indeed,  $\Phi(M)$ amounts to $F$.
%
It is easy to see that a logic program~$F$ can be identified with the \definition \mbox{$\defm{pred(F)}{F}$}. % as they have identical answer sets.
%When $F$ is 
%A standard logic program $F$ corresponds to a \definition \mbox{$\defm{pred(F)}{F}$} where all predicate symbols are intensional.
%
The \definition \mbox{$\defm{pred(F)}{F}$} assumes all predicate symbols in $F$ to be intensional.
If we leave some of them as extensional, then their extent is not ``minimized.''
%
For instance, an answer set of rule $\eqref{eq:hce1}$ alone -- \definition $\defm{edge,vertex}{\eqref{eq:hce1}}$ -- is empty; whereas in a \definition~$\defm{vertex}{\eqref{eq:hce1}}$
no assumption is made on extensional predicate $edge$, while $vertex$ collects precisely  all left arguments of $edge$.
%
% For simplicity, in the rest of the paper we will just identify each \definition $M$ with its SO-formula~$\Phi(M)$.

\black

A \emph{modular program} is a pair ${\mp = \tuple{\cS,\cM}}$ where $\cS \subseteq \cP$ is the set of \emph{public} predicate symbols and $\cM$ is the set of \emph{modules} $\{M_1,\dots,M_n\}$, where $M_i$ ($1\leq i\leq n$) is either a \emph{\definition} or another modular program (called  \emph{subprogram} of $P$), so that all predicate symbols occurring in $\mp$ are in $\cP$.
%
A modular program can be depicted as a hierarchical tree, whose leafs are \definitions.
%
%
The interpretation of a modular program $P=\tuple{\cS, \cM}$ is captured by the (recursively defined) formula:
$$
\Phi(\mp)
	\ \ \eqdef \ \ \exists \vec{h} \
\bigwedge_{M_i \in \cM}
\Phi(M_i),
$$
where $\vec{h}$ contains all free predicate symbols in $\Phi(M_i)$ that are not in $\cS$.
%
Notice that, if~$M_i$ is a \definition $\defm{\vec{p}}{F}$, then $\Phi(M_i)=\SM_\vec{p}[F]$ as we defined before, while if $M_i$ is a subprogram, we apply the formula above recursively.
%It is easy to see that if~$M_i$ is a \definition then all of its predicate symbols are public.
%
We say that an interpretation~$\cI$ is a \emph{model} of a modular program~$\mp$,
when it satisfies the formula~$\Phi(\mp)$.
As in the previous section,
we say that interpretation~$\cI$ over public predicate symbols $\cS$  is an \emph{answer set} of a modular program~$\mp$ when it is a Herbrand model of~$\mp$.
%
Under logic programming syntax (like Listing~\ref{list:hamiltonian}), public predicates are declared via {\tt \#show} clauses. % inside the module.
\red
When a modular program has a special form $\tuple{pred(F), \set{(\vec{p}:F)}}$, we identify it with  definition $(\vec{p}:F)$. 

\black
We define $\modules(P)$ as the set of all \definitions in $P$ at any level in the hierarchy.
%
\mbox{Program~$\mp=\tuple{\cS,\cM}$} is said to be \emph{flat} when it does not contain subprograms, i.e., $\cM$ coincides with $\modules(P)$.
%
We call flat modular program $\tuple{\cS,\cM}$ \emph{\mbox{HL-modular}}, when 
its set~$\cS$ of public predicates contains all predicate symbols occurring in $\cM$. HL-modular programs capture the definition of modular programs from~\citep{har16}.


We now illustrate a modular program that mimics 
encoding~$\fh$ (defined in Section~\ref{sec:sm}). % of the \hc derived from Listing~\ref{list:hamiltonian}.
% without {\tt \#show} statement. We construct an HL-modular program for this purpose.
This modular program comprises the same rules as~$\fh$
and has the same answer sets,
but
%Yet, unlike encoding~\eqref{eq:hc2} that only intuitively groups the rules,
adds explicit structure.
Each of its modules carries its own formal and intuitive meaning. 
The \hc modular program consists of  the following \definitions:
\begin{IEEEeqnarray}{lCCl}
( {\it vertex} & : & \eqref{eq:hce1} \wedge \eqref{eq:hce2} & \ ) \label{eq:hcmod1.1}\\
({\it in} & : & \eqref{eq:choicerulefo}& \ )
\label{eq:hcmod2}\\
({\it r}& : & \eqref{eq:hcr1} \wedge \eqref{eq:hcr2}& \ )
\label{eq:hcmod3}
\end{IEEEeqnarray}
%
%\begin{align}
% &\text{SM}_{{\it edge}}[{\it edge}(a, a')\wedge \;\; \dots \;\; \wedge {\it 
% edge}(c, c') ]\label{eq:hcmod1}\\
%&\begin{aligned}
%\text{SM}_{{\it vertex}}[&\forall x y(  {\it edge}(x,y)  \rar %{\it vertex}(x))\, \wedge\\
%&\forall x y(  {\it edge}(y,x)  \rar {\it vertex}(x))
%]
%\end{aligned}
%\label{eq:hcmod1.1}
%\\
%&\text{SM}_{{\it in}}[\forall x y(\neg \neg {\it in}(x,y) %\wedge {\it edge}(x,y) \rar {\it in}(x,y)]
%\label{eq:hcmod2}
%\\
%&
%\begin{aligned}
%\text{SM}_{{\it r}}[&\forall x y({\it in}(x,y) \rar {\it r}(x, %y)) \,\wedge\\
%\forall x y z({\it r}(x,z) \wedge {\it r}(z,y)\rar {\it %r}(x,y))]
%\end{aligned}
%\label{eq:hcmod3}
%\end{align}
%
together with formulas~\eqref{eq:hcmod4},~\eqref{eq:hcmod2.1}, and~\eqref{eq:hcmod2.2}.
%
\red
% This presentation is in spirit with the HL-modular program in~\citep{har16} given for the \hc encoding.
Observe how predicate symbol~$r$ only occurs in \definitions~\eqref{eq:hcmod2} and~\eqref{eq:hcmod4}.
%
We can hide this symbol from the rest of the modular program by encapsulating these two \definitions
in subprogram
\mbox{$
% \begin{gather}
    \mp_c = \tuple{\, \{ {\it vertex,\, in} \}, \{ \eqref{eq:hcmod3} ,\, \eqref{eq:hcmod4} \}\,}
%     \label{eq:modular.program.connected}
% \end{gather}
.$}
This subprogram corresponds to rules~4-6 in Listing~\ref{list:hamiltonian}
and intuitively states that relation~$in$ forms a strongly connected graph covering all vertices.
%
%The only public predicates of modular program $\mp_c$ are~${\it vertex} $ and  ${\it in}$.



\section{A formal specification language}
\label{sec:specification}
We follow the lines of~\cite{bre11} in stating  abstractly  what a search problem is.
A {\em search problem}~$\pi$ consists of a set of instances with each
{\em instance}~$I$ assigned a finite set~$\Theta_{\pi}(I)$ of solutions. 
In our use of modular programs as a formal specification language to capture a
search problem~$\pi$, we construct a modular program~$\mp_\pi$ that adheres to
problem specifications so that when extended with modular program $\mp_I$
representing an instance~$I$ of the problem, the answer sets of this join
are in one to one correspondence with members in~$\Theta_\pi(I)$.
%
In our methodology,
a formal specification for a search problem~$\pi$
is described as a modular program. 
%
Then, we can use this modular program to argue that each of its modules actually corresponds to some part of the informal description of the problem.
%
The interesting point is that this argument can be made in isolation: one module at a time.
%
We now illustrate these ideas on our running example.
%
For this purpose,
we consider the modular program
\begin{gather}
\mp_{\mathit{hs}} = \tuple{\, \set{\it edge,\, in},\,\set{ \eqref{eq:hcmod1.1}, \eqref{eq:hcmod2},\, \mh } \,}
\end{gather}
where 
${\mh = \tuple{\, \{ {\it vertex,\, in} \}, \{ \mp_c ,\, \eqref{eq:hcmod2.1} \}\,}}$
 (subprogram $\mp_c$ is defined in Section~\ref{sec:modlog}).
%
We argue that modular program~$\mp_{\mathit{hs}}$ is indeed a \emph{formal specification} for the search of \hcs.
%
%Note that this program does not contain any formula~\eqref{eq:hcmod2.2} as this is not necessary to capture the \hc problem.
%
% Note that~$\mp_c$ is a nested modular program itself.%
%
% We include proof sketches of the elements of this argument to illustrate how this methodology can be used in practice.
\black
%
We start by presenting the informal readings of all \definitions occurring in the program --- i.e., members of  $\modules(\mp_{\mathit{hs}})$.
The \definitions~\eqref{eq:hcmod1.1}-\eqref{eq:hcmod3} intuitively formulate the following {\em Statements}:
\begin{enumerate} 
\setlength\itemsep{0em}
% \item\label{l:item1}  An Herbrand {\it edge}-stable model of \definition~\eqref{eq:hcmod1} is any  Herbrand 
% interpretation $I$ over $\sigma(\mh)$ such that the extension\footnote{The {\sl extension} of a predicate in an interpretation is the set of 
% tuples that satisfy the predicate in that interpretation.} of the ${\it 
% edge}$ predicate in $I$ corresponds to the  facts in~\eqref{eq:hcfacts} (which encode a given graph). 
\item\label{l:item2}
In any model of~\eqref{eq:hcmod1.1},
the extent of ${\it vertex}$ corresponds to the objects  occurring in the extent of ${\it edge}$.

\item\label{l:item3}
In any model of~\eqref{eq:hcmod2},
the extent of ${\it in}$ is a subset of the extent of 
 ${\it edge}$. 
\item\label{l:item5} In any model of~\eqref{eq:hcmod3},
the extent of {\it r} is the transitive closure of the extent of {\it in}.
\end{enumerate}
These statements can be seen as {\em achievements} of each \definition in the sense of~\cite{lifschitz17a}.
%
Yet, these statements are agnostic to the context where \definitions appear.
%
This closely aligns with good software engineering practices, where the emphasis is made on modularity/independence of code development.
An intuitive meaning of formulas~\eqref{eq:hcmod4} and~\eqref{eq:hcmod2.1} is self explanatory given the underlying conventions of FO logic: %and translates into the following informal statements:
\begin{enumerate}
\setcounter{enumi}{3}
\item\label{l:hcmod4} In any model of~\eqref{eq:hcmod4},
the extent of ${\it r}$ contains each possible pair of vertices.
\item\label{l:hcmod2.1} In any model of~\eqref{eq:hcmod2.1},
the extent of ${\it in}$ does not contain two different pairs with the same left component.
% \item\label{l:hcmod2.2} In any model of~\eqref{eq:hcmod2.2},
% the extent of ${\it in}$ does not contain two different pairs with the same right component.
\end{enumerate}
Statements~\ref{l:item5} and~\ref{l:hcmod4} translate into a joint {\em Statement} about module $\mp_c$:
\begin{enumerate}
\setcounter{enumi}{5}
\item\label{l:hcmod7}
In any model of~$\mp_c$,
the extent of ${\it in}$ forms a strongly connected graph covering all vertices.
\end{enumerate}
\red
This plus Statement~\ref{l:hcmod2.1} lead to the following statement about subprogram~$\mh$,
\begin{enumerate}
\setcounter{enumi}{6}
\item\label{l:hcmod8}
In any model of~$\mh$,
the extent of ${\it in}$ is a \hc of the graph induced by its extent.
\end{enumerate}
%
Note that each subcomponent of the \hc modular program is small enough so that the verification of respective statements is a manageable and self-isolated task. 
%
In~\cite{cab20}, we use properties of the $\SM$ operator to provide formal proofs for the correctness of  Statements~\ref{l:item2}-\ref{l:hcmod2.1}.
In the sequel, we take their correctness for granted.
Here we showcase the formalization of Statement~\ref{l:item5}:
indeed, take $p$ and $q$ to be $\mathit{in}$ and~$\mathit{r}$, respectively, in the following.
%For instance, the following result formalizes Statement~\ref{l:item5}.
\black


\begin{proposition}[Theorem~3 in~\protected\citeNP{cab20}]
\label{prop:transitive.closure}
Let 
formula $F_{tr}^{qp}$ be 
\beq
\forall xy\big(p(x,y)\rar q(x,y)\big)\,\wedge
\forall xyz\big(q(x,z)\wedge q(z,y)\rar q(x,y)\big)
\eeq{eq:formulatheorem}
For any arbitrary predicates $p$ and $q$, any model $\cI$ of \definition 
$(q:F_{tr}^{qp})$
%${\text{\rm SM}}_{q}[F^{tr}_{qp}]$
is such that the    
the extent of {\it q} is the transitive closure of the relation constructed from the extent of~{\it p}.
\end{proposition}
% \begin{proofs}
% By Remark~1 from \citep{fer09}, we can replace the $\SM_q$ operator in
% ${\text{\rm SM}}_{q}[F^{tr}_{qp}]$
% by $\text{CIRC}_q$.
% %
% Each model of~$\hbox{CIRC}_{q}[F^{tr}_{qp}]$ is a model of~$F^{tr}_{qp}$ where the extent of~$q$ is minimal. Given FO formula $F^{tr}_{qp}$, this suffices to capture the transitive closure of the extent of~{\it p}.
% \end{proofs}
\red
%The semantics of \definition~\eqref{eq:hcmod3} is given by the SO formula 
%\mbox{$\text{SM}_{{\it r}}[  \eqref{eq:hcr1} \wedge \eqref{eq:hcr2}  ]$}.
%
%
% The rest of the modules admit similar proofs that we omit here for space reasons.
%
The proposition below states the correctness of Statements~\ref{l:hcmod7} and~\ref{l:hcmod8} about modular programs~$\mp_c$ and$\mh$. For an interpretation $\cI$ and a predicate symbol $p$, by $p^\cI$ we denote the extent of~$p$ in~$\cI$.  
\black

\begin{proposition}\label{prop:connectivity}
Let 
$F^{v}$ be formula
%\beq 
$\forall x y (  \neg{\it q}(x, y) \wedge {\it v}(x)\wedge 
{\it v}(y)\rar \bot)$; $F_{tr}^{qp}$ be formula~\eqref{eq:formulatheorem};
% \eeq{eq:formulatheorem2}
 $P_c^{vpq}$  
be a modular program $\tuple{\set{v,p}, \set{\,(q :F_{tr}^{qp}),\, F^v\,}}$; $\cI$ be an interpretation of $P_c^{vpq}$,
and
$\tuple{v^{\cI},p^{\cI}}$
be a graph.
%
Then, $\cI$ is a model of~$P_c^{vpq}$
iff 
for every pair \mbox{$a,b \in v^{\cI}$} of distinct vertices,
there is a directed path from~$a$ to~$b$ in $\tuple{v^{\cI},p^{\cI}}$.
\red

Furthermore, let $F^{p}$ be formula $\forall x y z({\it p}(x,y)\wedge {\it p}(x,z)\wedge \neg(y=z) \rar\bot)$, 
$\mh^{vpq}$ be modular program~$\tuple{\set{v,p}, \set{\, P_c^{vpq}, \, F^p \,}}$ and
$\cI$ be an interpretation of $\mh^{vpq}$.
Then, $\cI$ is a model of~$\mh^{vpq}$
iff $p^{\cI}$ are the edges of a Hamiltonian cycle of~$\tuple{v^{\cI},p^{\cI}}$
 that is,
% \begin{enumerate}
    % \item $V = \set{ a \mid (a,b) \in \mathit{in}^\cI } \cup \set{ b \mid (a,b) \in \mathit{in}^\cI}$
    % \item[]
    the elements of $\mathit{p}^\cI$ can be arranged as a directed cycle
    $(v_1,v_2),(v_2,v_3),\dots, (v_n,v_1)$
    so that $v_1,\dotsc,v_n$ are pairwise distinct
    and~$\mathit{v}^\cI=\{v_1,\dotsc,v_n\}$.
\end{proposition}

\begin{proofs}
We show here left to right direction
and the opposite direction is easy to check.
% The graph is connected iff, for every pair of vertices \mbox{$a,b \in v^{\cI}$},
% there is a directed path from $a$ to $b$.
% , that is, there is a subset $\set{a_0, \dotsc, a_n} \subseteq v^\cI$
% such that $a_0 = a$, $a_n = b$ and every $1 \leq i \leq n$,
% satisfies
% $(a_{i-1},a_{i}) \in p^\cI$.
Note first that $F^{v}$ is classically equivalent to  $\forall x y ( {\it v}(x)\wedge {\it v}(y)\rar {\it q}(x, y))$,
so any pair of vertices satisfies $(a,b) \in q^\cI$.
%
From Proposition~\ref{prop:transitive.closure},
relation~$q^\cI$ is the transitive closure of~$p^\cI$.
Hence,  path from $a$ to $b$  exists in graph $\tuple{v^{\cI},p^{\cI}}$.
%
\red

Furthermore,
if $\cI$ is a model of $\mh^{vpq}$,
the above implies
that for any pair \mbox{$v_1,v_m \in v^{\cI}$} of vertices,
there is a directed path
$(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1}, v_m)$
in  $\tuple{v^{\cI},p^{\cI}}$.
Hence,
there is a directed walk
\beq 
(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1},v_m),\allowbreak (v_{m+1},v_{m+1}),\dotsc,\allowbreak(v_n,v_1)
\eeq{eq:path}
in graph $\tuple{v^{\cI},p^{\cI}}$
such that  every vertex in $v^{\cI}$ appears in it.
%
Since $\cI$ is also a model of~$F^p$, Statement~\ref{l:hcmod2.1} (modulo names of predicate symbols) is applicable.
%
This implies $v_i \neq v_j$ for all $i \neq j$
and, thus, that all edges in~\eqref{eq:path} are distinct.
%
Therefore, \eqref{eq:path} is a directed cycle.
%
Since this cycle  covers all vertices of~$\tuple{v^{\cI},p^{\cI}}$,
 it is also a Hamiltonian cycle.
\end{proofs}

\noindent
Modular programs~$\mp_c$ and~$\mh$ coincide with modular programs
% \mbox{$\tuple{\set{v,p}, \set{\,(q : F^{tr}_{qp}),\, F_v\,}}$}
$\mp_c^{vpq}$ and~$\mh^{vpq}$
when  predicate symbols~$v$,~$p$ and~$q$ are replaced by~$\mathit{vertex}$, $\mathit{in}$ and~$\mathit{r}$, respectively.
%
Statements~\ref{l:hcmod7} and~\ref{l:hcmod8} follow immediately.
%
Note also that modular programs~$\mp_c$ and~$\mh$ also preserve their meaning inside a larger modular program mentioning predicate symbol~$r$ in other parts. Indeed, symbol $r$ is hidden or \emph{local} (existentially quantified) so that its use elsewhere in larger modular program has a different meaning.
%

To complete the modularization of the \hc problem, we develop  the encoding for a graph instance.
%
Given a set $E$ of graph edges,  $\mp_E$ denotes a \definition
%we define
\beq
% \begin{aligned}
\big(\, edge :  \bigwedge\set{\mathit{edge}(a,b) \mid (a,b) \in E} \,\big)
%\\
%M(E) \quad &\eqdef \quad \text{\normalfont SM}_{\mathit{edge}}[\mp_E]
% \end{aligned}
\eeq{eq:pe}
% and the \definition $M(E) \eqdef \text{\normalfont SM}_{\mathit{edge}}[\mp_E]$.
%
The intuitive and formal meaning of \definition  $\mp_E$  is captured by  {\em Statement}:
\begin{enumerate}
\setcounter{enumi}{7}
\item\label{l:hcmod9}
In any model of~$\mp_E$,
the extent of ${\it edge}$ coincides with set $E$ of edges.
\end{enumerate}

The \hc problem on a graph with edges~$E$
is encoded by modular program~$\mp_{\mathit{hs}}(E) = \tuple{ \, \set{\it in}, \, \set{ \mp_{\mathit{hs}} , \, \mp_E  } \, }$.
We now  state the result that pins the proposed methodology at work.
We show that modular program~$\mp_{\mathit{hs}}$ in fact reflects the \emph{informal description} of the \hc problem.
%
Thus,
we can use this modular program as a \emph{formal specification} of the problem.
%
In the next section,
we use $\mp_{\mathit{hs}}$ to \emph{verify} that the two logic programs for the \hc problem introduced in Section~\ref{sec:motivation} are correct.
Note that the proof of Proposition~\ref{prop:correct1} is obtained by combining the results corresponding to the submodules of program~$\mp_{\mathit{hs}}(E)$
--- we say submodules here to reflect on the fact that modular programs have recursive structure so that a module of a program may itself consist of modules and so forth.
%
For instance, we formalized
Statement~\ref{l:hcmod8} in Proposition~\ref{prop:connectivity} about submodule $\mh$ of program~$\mp_{\mathit{hs}}(E)$.
%
A similar proof at its full length is given at~\cite{cab20}; yet, in that paper HL-modular programs are used to capture the \hc problem.
%
That framework provides no account for {\tt \#show} statements and recursive submodules;
something that helped us simplifying the proof.
%
%
\black


\red

\begin{proposition}\label{prop:correct1}
Let $G = \tuple{V,E}$ be a graph with non-empty sets of vertices~$V$ and edges~$E$, where every vertex occurs in some edge, and~$\cI$ be an interpretation over signature~$\set{\mathit{in}}$.
Then,
$\cI$ is an answer set of~$\mp_{\mathit{hs}}(E)$ iff
$\mathit{in}^\cI$ is a \hc of $G$.
% \end{enumerate}
\end{proposition}

\begin{proofs}
% The proof is obtained by combining the results corresponding to all the modules of program~$\mp_{\mathit{hs}}(E)$, whose informal statements can be found above.
% %
% In particular,
% we have seen how statement~\ref{l:item6} was formalized in Proposition~\ref{prop:connectivity}.
% Note that any model~$\cI$ of \eqref{eq:hcmod1.1}-\eqref{eq:hcmod2}
% satisfies that~$\tuple{\vertex^\cI,\inp^\cI}$ is a subgraph of~$\tuple{\vertex^\cI,\edge^\cI}$
% (statements~\ref{l:item2}-\ref{l:item3}).
% Furthermore,
% from Proposition~\ref{prop:connectivity},
% for any model~$\cI$ of~$\mp_{\it c}$
% and any pair of vertices $v_1,v_n \in \vertex^\cI$,
% there is a directed path
% $(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1}, v_m)$.
% Hence,
% there is a directed path
% $(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1},v_m),\allowbreak (v_{m+1},v_{m+1}),\dotsc,\allowbreak(v_n,v_1)$.
% Finally, we can show that this is exactly the extension of  predicate~$\inp$.
% Any model of~$\mp_{\it c}$ that is also a model of~$\eqref{eq:hcmod2.1} \wedge \eqref{eq:hcmod2.2}$ and any vertex $v_i$ with $1 \leq i \leq n$ satisfies that
% $(v_{i-1},v_i)$ and $(v_i,v_{i+1})$,
% with $v_0 = v_{n+1} = v_1$,
% are the only pairs in $\inp^\cI$
% where $v_i$ occurs.
% As a result, we get $\vertex^\cI = \{v_1,\dotsc,v_n\}$
% and $\inp^\cI = \{ (v_1,v_2),\dots,(v_n,v_1) \}$.
% ================
We only showcase left to right direction.
Take interpretation $\cI$ to be an answer set of~$\mp_{\mathit{hs}}(E)$.
%
Then, there exists a Herbrand interpretation  
$\cJ$ over signature $in,vertex,edge$ so that
$\cJ$  coincides with~$\cI$ on the extent of $in$ and is a model of all submodules of $\mp_{\mathit{hs}}(E)$.
% namely,
% \eqref{eq:hcmod1.1}, \eqref{eq:hcmod2},\, $\mh$
% and~$\mp_E$.
%
Thus, 
$\cJ$  adheres to  Statements~\ref{l:item2},\ref{l:item3},\ref{l:hcmod8},\ref{l:hcmod9} about these submodules.
%
This implies that
the extent~$\mathit{in}^\cI$ forms a \hc of~$\tuple{\vertex^{\cJ},\inp^{\cJ}}$
(Statement~\ref{l:hcmod8})
and that $\tuple{\vertex^{\cJ},\inp^{\cJ}}$ is a subgraph of~$\tuple{\vertex^{\cJ},\edge^{\cJ}}$
(Statement~\ref{l:item3}).
%
Together, these two facts imply that~$\mathit{in}^\cI$ forms a \hc of the graph~$\tuple{\vertex^{\cJ},\edge^{\cJ}}$.
%
Moreover,
%
$\mathit{vertex}^{\cJ}$ and~$\mathit{edge}^{\cJ}$ respectively coincide with sets~$V$ and~$E$ (Statements~\ref{l:item2} and~\ref{l:hcmod8}).
%
Therefore,
~$\mathit{in}^\cJ$ forms a \hc of the graph~$\tuple{V,E} = G$.
%
Finally,
recall that
$\inp^{\cJ}=\inp^{\cI}$,
so the result holds.
%  Statements~\ref{l:hcmod2.1} and
% $\eqref{eq:hcmod2.1} \wedge $
%The other direction is easy to verify.
\end{proofs}





















\section{Verification based on modular programs}
\label{sec:verif}

In our methodology, \emph{verifying a logic program} means proving some form of equivalence between the program and its formal specification in the form of a modular program.
%
For instance, verifying the logic program in Listing~\ref{list:hamiltonian}
means proving that the answer sets of~$\fh$ and~$\mp_{hs}$ coincide.
% The ASP semantics is non-monotonic.
% %
% Thus, in general,
% the answer sets of modular program~$\tuple{\cS,\{ (\bp_1 : F_1 ) , \,  (\bp_2 : F_2 ) \}}$
% are not necessary the same as the answer sets of~$\tuple{\cS,\{ (\bp_1 \cup \bp_2 : F_1 \wedge F_2 ) \}}$.
% %
% % the conjunction of modules $\SM_{pred(F)}[F] \wedge \SM_{pred(F')}[F']$ is not equivalent to the whole program $\SM_\vec{p}[F \wedge F']$ for $\vec{p}=pred(F) \cup pred(F')$.
% %
% \sidecomment{This paragraph could be removed}
In the following, we present conditions under which the answer sets of a modular program coincide with the answer sets of its set of rules where the modular structure of a program is removed (conditions under which answer sets of, say, $\tuple{\cS,\{ (\bp_1 : F_1 ) , \,  (\bp_2 : F_2 ) \}}$
and~$\tuple{\cS,\{ (\bp_1 \cup \bp_2 : F_1 \wedge F_2 ) \}}$ coincide).
%

In the rest of the section,
we assume for simplicity that symbol $\mp$ denotes
an arbitrary modular program $\tuple{\cS,\cM}$.
% We say that modular program $\mp$ is \emph{flat} when~$\cM$ is a set of \definitions, that is, there are not nested modular programs in~$\cM$.
The \emph{flattening} of a modular program $P$ is defined as $\flatt{\mp} \eqdef \tuple{\cS,\modules(\mp)}$.
%
For example, 
$\flatt{\mp_{\mathit{hs}}(E)} = \tuple{\set{\it in},\set{ \eqref{eq:hcmod1.1},\allowbreak \eqref{eq:hcmod2},\allowbreak \eqref{eq:hcmod3},\allowbreak \eqref{eq:hcmod4} ,\allowbreak \eqref{eq:hcmod2.1},\allowbreak \eqref{eq:pe} }}$.
%where we recursively replace each subprogram by its \definitions.


We say that $\mp$ is in $\alpha$-\emph{normal form} (\ANF) if all occurrences of a predicate name in~$\Phi(\mp)$ are free or they are all bound to a unique occurrence of existential quantifier. For instance, $\mp_{\mathit{hs}}(E)$ is in \ANF{}.
%
Any formula $\Phi(\mp)$ can always be equivalently reduced to $\alpha$-NF by applying so-called $\alpha$-transformations (i.e., choosing new names for quantified variables).
%
In our context, this means changing hidden (auxiliary) predicate names in~$P$ until  \emph{different} symbols are used for distinct auxiliary predicates.
%
% Consider, modular program $P'_c$ that differs from $P_c$ in renaming its predicate symbol $r$ by $edge$; and
% modular program ${\mp_{\mathit{hs}}'}$ that differs from $\mp_{\mathit{hs}}$ by replacing module $P_c$ by $P'_c$. Program ${\mp_{\mathit{hs}}'}$
%  is not in \ANF{}. Yet,  it is 
%  equivalent to ${\mp_{\mathit{hs}}}$, since predicate symbol $edge$  is hidden within its submodule $P'_c$.
%
The next theorem states that, when modular program $\mp$ is in \ANF{}, we can ignore its recursive structure and instead consider its flat version.

\begin{comment}
\pedro{We can introduce the definition of \flattable in the proof of the theorem (perhaps as a lemma before, proving its relation to \ANF). But I found it too complicated for the main text.}
\emph{\flattable} if any modular program $\mp' \in \cM$ with $\mp' = \tuple{\cS',\cM'}$ satisfies the following conditions: 
\begin{enumerate}
\item 
predicate symbols occurring both in $\cS$ and $\mp'$ should also occur in $\cS'$,
    \label{item:flattable.2}
\item for any element (\definition or modular program) $M \in \cM$ different from  $\mp'$, 
if a predicate symbol~$p$ occurs in both $\mp'$ and $M$,
then $p \in \cS'$, and
    \label{item:flattable.1}

\item $\mp'$ is \flattable.
\end{enumerate}
\end{comment}

\begin{theorem}\label{thm:flatten}
For any modular program~$\mp$ in \ANF{}, an interpretation  $\cI$ is a model of $\mp$ iff $\cI$ is a model of $\flatt{\mp}$.
\end{theorem}
%
%Note that, in general, not every program is \flattable.
%
%In particular, this is not the case when the same predicate symbol is used locally in two different modules.
%
%Of course, the particular symbol that are used locally are not relevant for the semantics of a modular program.
%
%Hence,we can replace any local predicate symbol by a different predicate symbol and, thus, transform any non-\flattable a program into an equivalent \flattable one.

%{\color{green} YU: sections up to now fully reviewed. Few minor comments left for Jorge;
%Jorge, btw do you remember which problem Pedro suggested to model in addition to HC?
%} 

\red
This theorem affirms, for example,  the fact that program~$\mp_{\mathit{hs}}(E)$ is equivalent to flat modular program~$\flatt{\mp_{\mathit{hs}}(E)}$, where we understand the notion of equivalence between modular programs in a natural sense, i.e., modular programs are {\em equivalent} if they coincide on their models.
%

Next, we show  how to relate a flat program with a non-modular program that contains exactly the same rules. We use this result to verify that program in Listing~\ref{list:hamiltonian} satisfies the \hc specification.
\black
To formalize this relation we  focus on a syntax closer to one of logic programs. Consider FO formulas that are conjunctions of rules of the form:
% For HL-modular programs, \cite{har16} showed that there exists such a correspondence between the so called \emph{coherent} HL-modular programs and non-modular programs.
% In the rest of this section, we extend this correspondence to general case of modular programs defined here.
\beq
\ba{r}
\widetilde{\forall} (a_{k+1} \land \dots \land a_l \land \neg a_{l+1} \land \dots 
\land \neg a_m \,\land \neg \neg a_{m+1} \land \dots \land \neg \neg a_n \rar
a_1 
\lor \dots \lor a_k), 
\ea
\eeq{eq:rule_fo}
where all $a_i$ are atoms and $\widetilde{\forall}$ stands for the universal closure of their variables.
%
As usual, the consequent and the antecedent of~\eqref{eq:rule_fo} are  called {\em head} and  {\em body}, respectively.
%
The conjunction $a_{k+1} \land \dots \land a_{l}$ constitutes the {\em positive (part of the) body}.
%
A modular program~$\mp$ is called \emph{simple} if, for every \definition 
$({\bf p} : F) \in \modules(\mp)$, formula~$F$ is a conjunction of rules, and all head predicate symbols in $F$ are intensional (occur in~$\bf p$).
%
This is, in fact, the case of all \definitions we considered so far.
%For the remainder, we study the subclass of simple modular programs that help us connect  logic programs used in practice with a modular framework proposed here.
Let $\intens(\mp)$ collect all intensional predicates in $\mp$, that is $\intens(\mp) \eqdef \bigcup \{ \vec{p} \mid ({\bf p} : F) \in \modules(P)\}$.
%
Then, we form the directed \emph{dependency graph} $DG[\mp]$ by taking $\intens(\mp)$ as nodes and adding an edge $(p,q)$ each time there is a rule occurring in $\mp$ with $p$ in the head and $q$ is in the positive body. 
%
For instance, the dependency graph of program~$\mp_{\mathit{hs}}(E)$ is given in Figure~\ref{fig:example}~(Right).
%
This graph has four strongly connected components, each one consisting of a single node.
(In the sequel, we refer a dependency graph of a logic program. A logic program $F$ can be identified with modular program $\tuple{pred(F), \set{(pred(F):F)}}$.)

%
A modular program~$\mp$ is 
{\em coherent} if it is simple, in \ANF{}, and satisfies two more conditions: 
(i)  every pair of  distinct \definitions
 $({\bf p} : F)$
 and 
$({\bf p'} : F')$  in $\modules(\mp)$ is such that ${\bf p}~\cap~{\bf p'}~=~\emptyset$, 
and (ii)
 for every strongly connected component ${\tt SCC}$ in $DG[\mp]$, 
there is a \definition \hbox{$({\bf p} : F) \in \modules(\mp)$} such that ${\bf p}$ contains 
all vertices in~${\tt SCC}$.
%\end{enumerate}
For example, $\mp_{\mathit{hs}}(E)$ is a coherent program.
%
Now, let us collect the conjunction of all \definition formulas in $\mp$ as
$\formula(P) \eqdef \bigwedge \{F \mid ({\bf p} : F) \in \modules(\mp)\}.$
We can observe, for instance, that
$\fh \wedge \formula(P_E) = \formula(\mp_{\mathit{hs}}(E)) \wedge  \eqref{eq:hcmod2.2}  = \formula(\flatt{\mp_{\mathit{hs}}(E)}) \wedge  \eqref{eq:hcmod2.2} $, that is, the modular encoding of the \hc problem and the non-modular one share the same rules but for~\eqref{eq:hcmod2.2}.
%
We now obtain a similar result to Theorem~3 in~\citep{har16} but
extended to our framework.
%
Together with Proposition~\ref{thm:sm-traditional}, it connects modular programs with logic programs as used in practice.

\red
\begin{theorem}\label{thm:sm-traditional2.hidden}
Let $\mp = \tuple{\cS,\cM}$ be a coherent modular program, $\vec{p}$ be  $\intens(\mp)$, and $\vec{h}$ be $pred(\Phi(\mp))\setminus \cS$.
%
Then, (i) any interpretation~$\cI$ is a model of $\mp$ iff $\cI$ is a model of formula $\exists \bf h$ SM$_\vec{p}[\formula(\mp)]$; (ii)
any  interpretation~$\cI$ is an answer set of $\mp$ iff
 there is some answer set $\cJ$ of~$\formula(\mp)$ such that $\cI=\restr{\cJ}{\cS}$.
\end{theorem}


We use this result to prove that program in Listing~\ref{list:hamiltonian}  satisfies the formal specification~$\mp_{\mathit{hs}}$ of the \hc problem.
%
Therefore, this program also complies with the informal description of this problem as shown in the previous section.


\begin{proposition}
The answer sets of modular program~$\mp_{\mathit{hs}}(E)$
coincide with the answer sets of logic program $\fh \wedge\formula(P_E)$ for intensional predicate symbol $\mathit{in}$ hiding all other predicate symbols of the program.

%Modular program~$\mp_{\mathit{hs}}(E)$ has the same answer sets than~$\exists{\bf h} \text{SM}_\vec{p} [\fh \wedge\formula(P_E)]$
%for for any graph $G$ with edges $E$ (mentioning all vertices),
%where
\end{proposition}
\begin{proof}
Modular program~$\mp_{\mathit{hs}}(E)$ is coherent.
Theorem~\ref{thm:sm-traditional2.hidden} implies that~$\mp_{\mathit{hs}}(E)$ is equivalent 
to~\mbox{$\exists{\bf h} \text{SM}_\vec{p}[\formula(\mp_{\mathit{hs}}) \wedge \formula(P_E)]$} with hidden predicate symbols~\mbox{${\bf h}=\tuple{vertex,edge,r}$}.
This formula is equivalent 
to \mbox{$\exists{\bf h} \text{SM}_\vec{p}[\formula(\mp_{\mathit{hs}}) \wedge \eqref{eq:hcmod2.2} \wedge \formula(P_E) ]$}
since \mbox{$\formula(\mp_{\mathit{hs}})$} entails formula~\eqref{eq:hcmod2.2} and~\definition \eqref{eq:hcmod2.2} has no intensional predicate symbols.
In addition, formulas \mbox{$\formula(\mp_{\mathit{hs}}) \wedge \eqref{eq:hcmod2.2}$} and $\fh$ are identical.
From Proposition~\ref{thm:sm-traditional}, it follows that
 Herbrand models of~\mbox{$\exists{\bf h} \text{SM}_\vec{p}[\formula(\mp_{\mathit{hs}}) \wedge \formula(P_E)]$} are  answer sets of $\fh \wedge \formula(P_E)$ restricted to predicate~$in$.
\end{proof}

%As stated at the begining of the section,
%this result show that program in Listing~\ref{list:hamiltonian} complies with the formal specification~$\mp_{\mathit{hs}}$.
%
This proposition constitutes the verification step that links an ASP implementation of the \hc problem to its formal specification as a modular program $\mp_{\mathit{hs}}$.
%bmn 
% Proposition~\ref{prop:correct1} presented the claim of the correspondence between formal specification $\mp_{\mathit{hs}}$ and the informal description ofhjg the \hc problem.
Verifying the correctness of  program in Listing~\ref{list:hamiltonian} is a singular case since it contains almost the same rules as its formal specification modular program~$\mp_{\mathit{hs}}$.
%
In general, a program to be verified may contain different rules or even different  predicate symbols.
%
For instance, this is the case of the \hc program specified with the help of Listing~\ref{list:hamiltonian2}.
%
That program corresponds to the conjunction~$\fh'$ obtained from~$\fh$ by replacing
subformulas~\eqref{eq:hcr1}-\eqref{eq:hcmod4}
by
\begin{align}
&\forall y\big(\inp(a,y) \rar \rap(y)\big)
\label{eq:hcmod1.1a}
\\
&\forall x y \big(\inp(x,y) \wedge \rap(x)\rar \rap(y)\big) 
\label{eq:hcmod3.2b}
\\
&\forall y \big(\neg {\it ra}(y)\wedge {\it vertex}(y) \rar \bot\big)
\label{eq:hcmod4.2a}
\end{align}
Verifying  program $\fh'$ amounts to proving 
its adherence to~$\mp_{hs}$.
%
To this end, we transform~$\fh'$ into an equivalent modular program.

The definition of a coherent modular program lends itself to an intuitive procedure for  ``modularization'' of an arbitrary (non-modular) logic program. Intuitively, strongly connected components in the dependency graph
of a  logic program  suggest a way of partitioning its rules  into \definitions.
%
For instance, 
the modularization of logic program $\fh'$ 
results in a modular program
obtained from~$\mp_{\it hs}$ by replacing~$P_{\it hc}$ with~$Q_{\it hc}$,
where $Q_{\it hc} = \tuple{\set{\it vertex, in},\set{ Q_c, \eqref{eq:hcmod2.1}, \eqref{eq:hcmod2.2} }}$ and
$Q_{\it c} = \tuple{\set{\it vertex, in},\set{ (ra: \eqref{eq:hcmod1.1a}\wedge\eqref{eq:hcmod3.2b}),\eqref{eq:hcmod4.2a} }}$.
We call this program $\mp'_{\it hs}$.
%and
%\begin{align}
%&\begin{aligned}
%\big( {\it \rap} & : & \forall y\big(\inp(a,y) \rar \rap(y)\big) \,\wedge%\\
%%&
%\forall x y \big(\inp(x,y) \wedge \rap(x)\rar \rap(y)\big) &  \big)\\
%\end{aligned}
% \label{eq:hcmod1.1}
%\label{eq:hcmod3.2}
%\\
%&\forall y \big(\neg {\it ra}(y)\wedge {\it vertex}(y) \rar \bot\big)
%\label{eq:hcmod4.2}
%\end{align}
The intuitive meaning of $Q_{\it hc}$ and $P_{\it hc}$ coincide as long as vertex $a$ is present in larger context (despite their differences in the use of auxiliary predicates). 
%:the extent of~$in$ forms a strongly connected graph covering all vertices.
This strong relation between these modular programs suggests that we can often use them interchangeably as they ensure the same property. 
Now, we show now how to formally relate these two modular programs.




%\paragraph{Equivalent modular programs.}
Given modular programs~$\mp,\mp_1$ and $\mp_2$, we write $\mp[\mp_1/\mp_2]$ to denote the result of replacing all occurrences of module~$\mp_1$ in~$\mp$ by $\mp_2$.
%
We also define $\Phi(\mp-\mp_1) \eqdef \bigwedge \{\Phi(M) \mid M \in \cM, P_1 \not\in \modules(M) \} $.
%
For any theory $\Gamma$, two modular programs~$\mp_1$ and~$\mp_2$ are said to be \emph{strongly equivalent with respect to context~$\Gamma$} when any modular program~$\mp$ with $\Phi(\mp - \mp_1) \models \Gamma$
satisfies that $\mp$ and~$\mp[\mp_1/\mp_2]$ have the same answer sets.
%
%We say that ~$\mp_1$ and~$\mp_2$ are just \emph{strongly equivalent} when they are strongly equivalent
%under the empty context~$\emptyset$.

%Formally, given modular programs~$\mp,\mp'$ and $\mp''$, we write $\mp''[\mp/\mp']$ to denote the result of replacing all occurrences of the module~$\mp$ in~$\mp''$ by $\mp'$.
%
%Furthermore, assuming that $\mp''$ is of the form $\tuple{\cS'',\cM''}$, we also define $\modules(\mp'' - \mp) \eqdef \set{ M \in \cM'' \mid \mp \notin \modules(M) }$
%
%We say that two modular programs~$\mp$ and~$\mp'$ are \emph{strongly equivalent with respect to some context~$\Gamma$} when any modular program~$\mp''$ with  $\bigwedge \modules(\mp'' - \mp) \models \Gamma$ satisfies that $\mp''$ and~$\mp''[\mp/\mp']$ have the same answer sets.
%
%We say that ~$\mp$ and~$\mp'$ are \emph{strongly equivalent} when they are strongly equivalent with respect to~$\emptyset$.

\begin{theorem}
\label{thm:modular.equivalence}
Two modular programs~$\mp$ and~$\mp'$ are strongly equivalent under context~$\Gamma$ iff
\mbox{$\Gamma \models \Phi(\mp) \leftrightarrow \Phi(\mp')$} holds in SO logic.
\end{theorem}

% \begin{proof}
% Let $\mp'' = \tuple{\cS,\cM}$ be a modular program such that
% $\bigwedge \modules(\mp'' - \mp) \models \Gamma$.
% Note that, by definition,
% \mbox{$\Phi(\mp'') \leftrightarrow \Phi(\mp''[\mp/\mp'])$}
% implies that 
% $\Phi(\mp'')$
% and
% $\Phi(\mp''[\mp/\mp'])$
% have the same models
% and, thus,
% that~$\Phi(\mp'')$ and~$\Phi(\mp''[\mp/\mp'])$
% are strongly equivalent with respect to~$\Gamma$.
% %
% Assume that~$\mp''[\mp/\mp'] = \tuple{\cS,\cM'}$
% and let
% $\cM_1 = \modules(\mp'' - \mp)$
% and~$\cM_2 = \cM \setminus \cM_1$
% be sets of modules.
% Then, 
% $\cI \models \Phi(\mp'') = \exists \vec{h} \ \bigwedge \cM$
% iff
% $\cI \models  \exists \vec{h} \ (\bigwedge \cM_1 \wedge \bigwedge \cM_2)$
% iff
% $\cI \models  \exists \vec{h} \ (\bigwedge \cM_1 \wedge \bigwedge \set{ M[\mp/\mp'] \mid \mp \in \cM_2 })$
% iff
% \mbox{$\cI \models \Phi(\mp''[\mp/\mp'])$}.
% \end{proof}
\red
Back to our example,
we can see that, even though
$\Phi(\mp_{\it hc})$ and $\Phi(Q_{\it hc})$
are not in general equivalent,
they are strongly equivalent in context of the programs~$\mp_{\mathit{hs}}(E)$ and~$\mp'_{\it hs}(E)$ when a given graph has a vertex named $a$.

\begin{proposition}\label{prop:ham.equivalence}
Modules $\mp_{\it hc}$ and~$Q_{\it hc}$
are strongly equivalent w.r.t.~$\set{ \vertex(a) }$.
\end{proposition}
\begin{proofs}
Recall that
\mbox{$\mp_{\it hc} \models\eqref{eq:hcmod2.2}$}.
The rest of proof consists of two steps.
%
First, given:
\begin{align}
&\exists r\, \big(\ \Phi\eqref{eq:hcmod3} \wedge \forall y (\vertex(a)\wedge\vertex(y)  \rar \rp(a,y)) \ \big)
\label{eq:hcmod4.4}
\end{align}
we prove that 
\mbox{$\vertex(a) \models \Phi(Q_{\it c}) \leftrightarrow \eqref{eq:hcmod4.4} $}
and, furthermore, that
$\models \Phi(\mp_{\it c}) \to \eqref{eq:hcmod4.4}$
follows by instantiation of~$\forall x$ with \mbox{$x=a$}.
%
Second, we prove 
\mbox{$\eqref{eq:hcmod2.1} \models \eqref{eq:hcmod4.4} \to \Phi(\mp_{\it c})$}.
\end{proofs}

%This result immediately implies that the answer sets of logic program $\fh$ for intensional predicate symbol $\mathit{in}$ hiding all other predicates of the program coincide with the answer sets of the specification~$\mp_{\mathit{hs}}$ for any graph.


% \begin{proposition}
% Let $\cI$ be some interpretation satisfying 
% the fact $vertex(a)$
% and the formula~$\eqref{eq:hcmod2.1}$.
% Then,
% $\cI$ is a model of~$\mp_{\it c}$
% iff
% $\cI$ is a model of~$Q_{\it c}$.
% \end{proposition}



==> background.tex <==
%!TEX root = verification-modular-show.tex



\section{Operator SM with hidden predicates}\label{sec:sm}

Answer set semantics is nowadays defined for arbitrary first-order (FO) theories thanks to the introduction of \emph{Quantified Equilibrium Logic}~\cite{peaval06a} and its equivalent formulation using the second-order (SO) operator {SM}~\cite{fer09}.
%
These approaches allow us to treat program rules as logical sentences and assigning them a meaning that bypasses grounding.
%
For instance, the rules in Listing~\ref{list:hamiltonian} respectively correspond to the following sentences:
\begingroup
\allowdisplaybreaks
\begin{align}
% &{\it edge}(a, a')\wedge \;\; \dots \;\; \wedge {\it edge}(c, c') \; \\
&\forall x y({\it edge}(x,y) \rar {\it vertex}(x)) \; \label{eq:hce1}\\
&\forall x y({\it edge}(y,x) \rar {\it vertex}(x)) \; \label{eq:hce2}\\
&\forall x y( \neg\neg  {\it in}(x,y) \wedge {\it edge}(x,y) \rar {\it 
in}(x,y)) \; \label{eq:choicerulefo}\\
&\forall x y({\it in}(x,y) \rar {\it r}(x, y)) \; \label{eq:hcr1}\\
&\forall x y z({\it r}(x,z) \wedge {\it r}(z,y)\rar {\it r}(x,y)) \; \label{eq:hcr2}
\\
&\forall x y (\neg {\it r}(x, y)\wedge {\it vertex}(x)\wedge {\it 
vertex}(y)\rar \bot) \label{eq:hcmod4}\\
&\forall x y z({\it in}(x,y)\wedge {\it in}(x,z)\wedge \neg(y=z) \rar\bot) 
\; \label{eq:hcmod2.1}\\
&\forall x y z({\it in}(x,z)\wedge {\it in}(y,z)\wedge \neg(x=y) \rar\bot) 
\; \label{eq:hcmod2.2} 
\end{align}
\endgroup
We name the conjunction of sentences~\eqref{eq:hce1}-\eqref{eq:hcmod2.2}  as $\fh$. 
%
The correspondence of these sentences to program's rules is straightforward except, perhaps, for the \emph{choice} rule in line~3
%\begin{verbatim}
% {\tt \{ in(X,Y) \}:- edge(X,Y).}    
%\end{verbatim}
% \noindent
of Listing~\ref{list:hamiltonian} that is represented as formula~\eqref{eq:choicerulefo} (see~\citeNP{fer05} for more details).
% showed that a choice  rule can be seen as an abbreviation for a formula that uses doubly negated atoms as illustrated by our example.


%
We now recall the SM operator as defined in~\cite{fer09} and then introduce its slight variation to ``remove'' some predicate symbols from its models.
%
We assume familiarity with second order (SO) logic.
% \jcomment{(see~\ref{?????} for more details)}.
% We start this section by reviewing the second order logic. We then review the SM operator.
% \input{so.tex}
% \subsection{Operator SM}\label{sec:sm}
% We are now ready to introduce the operator SM by~\cite{fer09}.
%
We adopt some notation: letters in boldface inside formulas denote tuples of elements.
%
When a tuple is formed by different variable names, we sometimes use it as a set.
%
Quantifiers with empty tuples (or empty sets of variables) can be removed: $\exists \emptyset F = \forall \emptyset F := F$.
%
Expression $pred(F)$ stands for the set of free predicate names in a SO formula $F$.
%
If $p$ and $q$ are predicate symbols (constants or variables) of the same arity~$m$ then $p \leq q$ is an 
abbreviation of the formula 
$
\forall {\bf x}(p({\bf x}) \rar q({\bf x})), 
$
where ${\bf x}$ is an $m$-tuple of \mbox{FO variables}. If ${\bf p}$ and ${\bf 
q}$ are tuples $p_1, \dots, p_n$ and $q_1, \dots, q_n$ of predicate symbols, then 
${\bf p} \leq {\bf q}$ is an abbreviation of the conjunction 
$
(p_1 \leq q_1) \land \dots \land (p_n \leq q_n),
$ 
and 
${\bf p} < {\bf q}$ is an abbreviation of 
$({\bf p} \leq {\bf q}) \land \neg ({\bf q} \leq {\bf p})$.
If ${\bf p}$ is a tuple of predicate symbols $p_1, \dots, p_n$
(not including equality) and $F$ 
is a FO formula 
then SM$_{\bf p}[F]$
(called the {\em stable model operator with intensional predicates ${\bf p}$})
denotes the SO formula 
\begin{equation}
F \land \neg \exists {\bf u}\big( \ ({\bf u} < {\bf p}) \land F^*({\bf u})\ \big), \label{f:sm}
\end{equation}
where ${\bf u}$ is a tuple of distinct predicate variables $u_1, \dots, u_n$ not occurring in ${\bf p}$, and $F^*({\bf u})$ is defined recursively:
%\vspace{-.3cm}
\begin{itemize}
\setlength\itemsep{0em}
% \item $\bot^*$ is $\bot$;
% \item $(t_1 = t_2)^*$ is $(t_1 = t_2)$ for any terms $t_1, t_2$;
\item $F^*$ is $F$ for any atomic formula $F$ that does not contain members of 
$\bp$;%\footnote{This includes equality statements and the formula $\bot$.} 
\item $p_i({\bf t})^*$ is $u_i({\bf t})$ for any tuple ${\bf t}$ of terms;

\item $(F \land G)^*$ is $F^* \land G^*$;
\item $(F \lor G)^*$ is $F^* \lor G^*$;
\item $(F \rar G)^*$ is $(F^* \rar G^*) \land (F \rar G) $;
\item $(\forall x F)^*$ is $\forall x F^*$;
\item $(\exists x F)^*$ is $\exists x F^*$.
\end{itemize}
Predicate symbols occurring in $F$ but not in $\vec{p}$ are called \emph{extensional} and are interpreted classically.
%
In fact, if ${\bf p}$ is empty, it is easy to see that SM$_{\bf p}[F]$ coincides with $F$.
%
Operator $\SM_\vec{p}[F]$ is formally similar to circumscription  $\text{CIRC}_\vec{p}[F]$: in fact, the latter amounts to replacing $F^*(\vec{u})$ by $F(\vec{u})$ in \eqref{f:sm}.
%
We say that an interpretation~$\cI$ over a signature~$\cP$ is an \emph{answer set} of a FO formula~$F$ (representing a logic program) when it is a Herbrand model of
SM$_\vec{p}[F]$ and $\vec{p}=pred(F)$.
%
When $F$ is a logic program, answer sets defined in this way correspond to the traditional definition based on grounding~\cite{fer09}.
It is common to identify Herbrand interpretations with sets of atoms
corresponding to its predicates and their extensions (the {\em extension} or {\em extent} of a predicate in an interpretation is the set of tuples that satisfy the predicate in that interpretation). Here, we often adopt this convention.

%


As a small example, let $F_g$ be the conjunction of facts in Listing~\ref{list:graph1}. Let $F_1$ denote a conjunction of  $F_g$ and $\eqref{eq:hce1}$.
%
%The predicates in $F_1$ are $\vec{p}=\tuple{edge,vertex}$. 
Let $\vec{u}$ be $\tuple{e,v}$. Then, $F_1^*(\vec{u})$ is formed as a conjunction of formula
$
\forall x y ( (e(x,y) \to v(x)) \wedge (edge(x,y) \to vertex(x)))
$
and atoms $e(x,y)$ per each fact $edge(x,y)$ in $F_g$.
%
The answer sets of $F_1$ are captured by the Herbrand models of 
$$
\text{SM}_{\tuple{edge,vertex}}[F_1] = F_1 \wedge \neg \exists e v \big (\tuple{e,v} < \tuple{edge,vertex} \wedge F_1^*(\vec{u}) \big)
$$
This formula has a unique model that minimizes the extension of $edge$ to the exact set of facts in $F_g$ (and not more) and the extension of $vertex$ to be precisely all nodes used as left arguments in those edges.
%
If we take instead  program $F_2:=\fh \wedge F_g$
so that $\vec{p}_2$ denotes all predicates in $F_2$ then 
\mbox{SM$_{\vec{p}_2}[F_2]$}
has a unique Herbrand model whose  ${\it in}$ atoms coincide with these listed in Listing~\ref{list:answer} but, obviously, this model has more atoms for the remaining predicates in the formula's signature. %, including the auxiliary atoms of the form $r(\cdot,\cdot)$.
%
To ``remove'' those extra predicates, we  convert them into existentially quantified predicate variables.
%
Given formula $F$ and tuples of predicate symbols $\vec{p}$ and~$\vec{h}$, we define the \emph{answer sets of~$F$ for $\vec{p}$ hiding $\vec{h}$} as the Herbrand models of the formula:
\begin{equation}
\exists \vec{h} \ \text{SM}_\vec{p}[F] \label{f:hSM}
\end{equation}
We call predicates in tuples $\vec{p}$ and  $\vec{h}$ {\em intensional} and {\em hidden}, respectively.
For instance, formula
$\exists \mathit{edge} \, \mathit{vertex} \, \mathit{r}\  \text{SM}_{\vec{p}_2}[F_2]$
has a unique Herbrand model that coincides with the one in Listing~\ref{list:answer}.
Thus, this model forms the unique answer set of $F_2$ for $\vec{p}_2$ hiding 
$\mathit{edge} \, \mathit{vertex} \, \mathit{r}$.
%
This corresponds to the behavior produced by the~$\tt \#show$ directive in Line~9 of the \hc encoding.
% Listing~\ref{list:answer1}.
\begin{comment}
At the same time, it is safe to rewrite~\eqref{eq:choicerulefo} as follows 
$$
\forall x y(  {\it edge}(x,y)) \rar {\it 
in}(x,y) \vee \neg  {\it in}(x,y)).
$$
The last formula may provide a better insight to an intuitive meaning of this rule. Yet, for the later presentation it is convenient for us to use the presentation of a choice rule exemplified in~\eqref{eq:choicerulefo}. 
\end{comment}
%
%

For a Herbrand interpretation $\cI$ over set~$\cP$ of predicates  and set $\cS\subseteq\cP$, we write  $\restr{\cI}{\cS}$ to denote the restriction of $\cI$ to $\cS$.
%
The following proposition states that the existential quantifiers for hidden predicates filter out their information in the models.

\begin{proposition}\label{thm:sm-traditional}
Let $F$ be a formula, $\vec{h}$ a tuple of predicate symbols from $F$ and let
\mbox{$\cS=pred(F) \setminus \vec{h}$}.
%
Then, $\cI$ is a Herbrand model of \eqref{f:hSM} iff there is some answer set $\cJ$ of~$F$ such that $\cI=\restr{\cJ}{\cS}$.
\end{proposition}
%
Rewriting auxiliary predicate symbols as existentially quantified predicate variables 
makes names of these hidden symbols immaterial: they can be arbitrary renamed.


==> conlcusions.tex <==
\black
\section{Conclusions and future work}
\label{sec:conc}
We  presented a modular ASP framework that allows nested modules possibly containing hidden local predicates.
%
The semantics of these programs and their modules is specified via  the second-order SM operator, and so, it does not resort to grounding.
%
We  illustrated how, under some reasonable conditions, a modular reorganization of a logic program can be used for verifying that it adheres to its (in)formal specification.
%
This method has two important advantages.
%
First, it applies a divide-and-conquer strategy, decomposing the correctness proof for the target program into almost self-evident pieces.
%
Second, it can be  used to guarantee correctness of a module replacement, even if interchanged modules are non-ground and use different local predicates.
%
Due to
the use of second-order logic we lack a proof theory in the general case. Yet, 
there are well-known specific cases in which the second-order quantifiers can be removed.
%
This is often the case of the SM operator
so that we can use formal results from the literature (splitting, head-cycle free transformations, relation to Clark's Completion or Circumscription -- see \citep{fer09})  to reduce the these second-order formulas to first-order ones.
%
We intend to exploit the correspondence between SM and Equilibrium Logic to study more general inter-theory relations~\cite{PV04}.
%
\red
It is also worth  mentioning that since verification happens at the level of modules,
the formal statements about these modules can be reused when they occur in a different program.
%
This essentially means that modules have to be verified once: the reusability of those modules comes accompanied by the reusability of their formal results.
\black

Our definition of contextual strong equivalence using hidden predicates is a generalization of \emph{strong equivalence}~\cite{lipeva01a,lif07a} and \emph{projective strong equivalence}~\cite{AguadoCFPPV19}.
%
We leave it to future work the relation to other generalizations of strong equivalence~\cite{eitowo05a,OikarinenJ09,GeibingerT19}.
%
% Another interesting future direction is establishing a formal connection to the modular approach in~\cite{oikjan06a} and, especially, the removal of local auxiliary predicates through \emph{forgetting}~\cite{goncalves19}.
%
% An important difference with our proposal is that these approaches rely on the program grounding.
%
Another topic for future work is the extension of automated reasoning tools for ASP verification~\cite{lifschitz18a} to incorporate modularity. It is also interesting to explore the generalization of this framework to richer fragments of ASP that may contain aggregates or numerical constraints.



\begin{comment}

--------------------------------------------------

Obviously, the semantics of a module is given by a SO formula, which at times is complex for providing intuitive arguments about its formulas. Yet, here we are able to construct an intuitive justification 
about  the correspondence of a module and its informal meaning. In this construction, we rely on the relation between minimal models of a FO formula of a module and its formal SO semantics.
%
%In other cases, similar arguments 
%rely on the relation between the completion~\cite{cla78} of a FO formula corresponding to a module and its formal SO semantics.
% (The notion of program's completion was first introduced in.)
%
Note that, given the modular nature of our approach,
the conditions necessary to reduce the SM operator to a simpler formalism are checked in each module rather than on the whole program.
%
In this sense,
we may expect that  modules can often be reduced either to circumscription or completion of FO formulas.


% --------------------------------------
\end{comment}


% In general,
% this equivalence needs to account for the possible use of different auxiliary predicates in the formal specification and the program to be verified~\cite{ETW05,AguadoCFPPV19,GeibingerT19}
% or the fact that input of the program consists exclusively of facts~\cite{eitfin03a,EiterFTW05}.

==> equivalence.tex <==
\section{Equivalent modular programs}
\label{sec:eqp}

\red
Verifying the correctness of the \hc program in Listing~\ref{list:hamiltonian} is a  singular case since it contains exactly the same rules as its formal specification  -- modular program~$\mh^m(E)$.
%
In general, a program to be verified may contain different rules or even different  predicate symbols.
%
For instance, this is the case of the \hc program specified with the help of  Listing~\ref{list:hamiltonian2}.
We now show how modular program approach provides us with convenient means for arguing correctness of a less straightforward encodings of a given problem. 

The definition of a coherent modular program lends itself to an intuitive procedure for  ``modularization'' of an arbitrary (non-modular) logic program. Intuitively, strongly connected components in the dependency graph
of a  logic program  suggest a way of partitioning its rules  into \definitions.
%
For instance, 
the modularization of the \hc program stemming from Listing~\ref{list:hamiltonian2}
results in  modular program
$Q^m_{\it hc}$ 
%= \tuple{\, \set{\it edge,\, in},\,\set{ \eqref{eq:hcmod1.1}, \eqref{eq:hcmod2},\, Q_c\, , \eqref{eq:hcmod2.1}, \eqref{eq:hcmod2.2} } \,}$.
% where~$Q_c$ is in its turn the modular program corresponding to the rules in Listing~\ref{list:hamiltonian2}.
% %
% That is,
% $Q_{\it c} = \tuple{\set{\it vertex, in},\set{ \eqref{eq:hcmod3.2},\eqref{eq:hcmod4.2} }}$ with \definitions:
% \begin{align}
% &\begin{aligned}
% \text{SM}_{\rap}[&\forall y(\inp(a,y) \rar \rap(y)) \,\wedge\\
% &\forall x y (\inp(x,y) \wedge \rap(x)\rar \rap(y))]
% \end{aligned}
% \label{eq:hcmod3.2}
% \\
% &\forall y (\neg {\it ra}(y)\wedge {\it vertex}(y) \rar \bot)
% \label{eq:hcmod4.2}
% \end{align}
 obtained from~$P^m_{\it hc}$ by replacing~$P_c$ with~$Q_c$ (defined in Section~\ref{sec:modlog}).
%
Thus, checking that the program corresponding to~Listing~\ref{list:hamiltonian2} satisfies the specification~$P^m_{\it hc}$ is reduced to 
checking that it is ``safe'' to replace~$P_c$ by~$Q_c$ within $P^m_{\it hc}$. In the following, we make the notion of safe replacement precise.
\begin{comment}
%% YU: the narrative below is commented out as it requires careful revision. Possibly paper is OK without it 
%
In general, varying a non-modular program can be reduced to check some kind of \emph{strong equivalence} between the different modules of both program~\cite{lipeva01a,lif07a}.
%
This equivalence needs to account for the possible use of different auxiliary predicate symbols in both modules~\cite{ETW05,AguadoCFPPV19,GeibingerT19}
and the modular structure of the program~\cite{OikarinenJ09}.
%
However,
even taking into account these two notions is not always enough.
%
As an example, 
modules~$P_c$ and~$Q_c$ are not equivalent for they public predicate symbols in every context,
though they can be safely replaced one by the other in this context.
%
In the following,
we describe a form of strong equivalence that takes into account both the public predicate symbols and the context in which the replacement can safely be made.
\end{comment}
\black
% In other words, we proved correctness of program $\fh$ (i.e., Listing~\ref{list:hamiltonian}) by resorting to the correctness of its modularization $\mh^m$ (Proposition~\ref{prop:correct1}).
% %
% The interest of this modular method is not only breaking the proof into smaller and simpler pieces, but also that, once we identify program fragments with an independent meaning, it is easy to make a \emph{correct local replacement} by alternative code.
% %
% For instance, once we spotted that rules~3-5 in Listing~\ref{list:hamiltonian} formally express that our solutions in terms of $in$ are strongly connected (statement~\ref{l:item6} for subprogram $P_c$) we can now consider replacing those rules by Listing~\ref{list:hamiltonian2}, as we suggested in the introduction.
% %
% To do so, take 
% %
% Then, we only need to prove that modules~$\mp_{\it c}$ and $Q_{\it c}$ are equivalent in this context.

Given modular programs~$\mp,\mp_1$ and $\mp_2$, we write $\mp[\mp_1/\mp_2]$ to denote the result of replacing all occurrences of module~$\mp_1$ in~$\mp$ by $\mp_2$.
%
We also define $\Phi(\mp-\mp_1) \eqdef \bigwedge \{\Phi(M) \mid M \in \cM, P_1 \not\in \modules(M) \} $.
%
For any theory $\Gamma$, two modular programs~$\mp_1$ and~$\mp_2$ are said to be \emph{strongly equivalent with respect to context~$\Gamma$} when any modular program~$\mp$ with $\Phi(\mp - \mp_1) \models \Gamma$
satisfies that $\mp$ and~$\mp[\mp_1/\mp_2]$ have the same answer sets.
%
%We say that ~$\mp_1$ and~$\mp_2$ are just \emph{strongly equivalent} when they are strongly equivalent
%under the empty context~$\emptyset$.

%Formally, given modular programs~$\mp,\mp'$ and $\mp''$, we write $\mp''[\mp/\mp']$ to denote the result of replacing all occurrences of the module~$\mp$ in~$\mp''$ by $\mp'$.
%
%Furthermore, assuming that $\mp''$ is of the form $\tuple{\cS'',\cM''}$, we also define $\modules(\mp'' - \mp) \eqdef \set{ M \in \cM'' \mid \mp \notin \modules(M) }$
%
%We say that two modular programs~$\mp$ and~$\mp'$ are \emph{strongly equivalent with respect to some context~$\Gamma$} when any modular program~$\mp''$ with  $\bigwedge \modules(\mp'' - \mp) \models \Gamma$ satisfies that $\mp''$ and~$\mp''[\mp/\mp']$ have the same answer sets.
%
%We say that ~$\mp$ and~$\mp'$ are \emph{strongly equivalent} when they are strongly equivalent with respect to~$\emptyset$.

\begin{theorem}
\label{thm:modular.equivalence}
Two modular programs~$\mp$ and~$\mp'$ are strongly equivalent under context~$\Gamma$ iff
\mbox{$\Gamma \models \Phi(\mp) \leftrightarrow \Phi(\mp')$} holds in SO logic.
\end{theorem}

% \begin{proof}
% Let $\mp'' = \tuple{\cS,\cM}$ be a modular program such that
% $\bigwedge \modules(\mp'' - \mp) \models \Gamma$.
% Note that, by definition,
% \mbox{$\Phi(\mp'') \leftrightarrow \Phi(\mp''[\mp/\mp'])$}
% implies that 
% $\Phi(\mp'')$
% and
% $\Phi(\mp''[\mp/\mp'])$
% have the same models
% and, thus,
% that~$\Phi(\mp'')$ and~$\Phi(\mp''[\mp/\mp'])$
% are strongly equivalent with respect to~$\Gamma$.
% %
% Assume that~$\mp''[\mp/\mp'] = \tuple{\cS,\cM'}$
% and let
% $\cM_1 = \modules(\mp'' - \mp)$
% and~$\cM_2 = \cM \setminus \cM_1$
% be sets of modules.
% Then, 
% $\cI \models \Phi(\mp'') = \exists \vec{h} \ \bigwedge \cM$
% iff
% $\cI \models  \exists \vec{h} \ (\bigwedge \cM_1 \wedge \bigwedge \cM_2)$
% iff
% $\cI \models  \exists \vec{h} \ (\bigwedge \cM_1 \wedge \bigwedge \set{ M[\mp/\mp'] \mid \mp \in \cM_2 })$
% iff
% \mbox{$\cI \models \Phi(\mp''[\mp/\mp'])$}.
% \end{proof}
\red
Back to our example,
we can see that, even though
$\Phi(\mp_{\it c})$ and $\Phi(Q_{\it c})$
are not in general equivalent,
they still are equivalent in context of the programs~$P^m_{\it hc}$ and~$Q^m_{\it hc}$ when a given graph has a vertex named $a$.

\begin{proposition}\label{prop:ham.equivalence}
Modules $\mp_{\it c}$ and~$Q_{\it c}$
are strongly equivalent w.r.t.~$\set{ \vertex(a), \eqref{eq:hcmod2.1} }$.
\end{proposition}
\begin{proofs}
The proof consists of two steps.
%
First, given:
\begin{align}
&\exists r\, \big(\ \eqref{eq:hcmod3} \wedge \forall y (\vertex(a)\wedge\vertex(y)  \rar \rp(a,y)) \ \big)
\label{eq:hcmod4.4}
\end{align}
we prove that 
\mbox{$\vertex(a) \models \Phi(Q_{\it c}) \leftrightarrow \eqref{eq:hcmod4.4} $}
and, furthermore, that
$\models \Phi(\mp_{\it c}) \to \eqref{eq:hcmod4.4}$
follows by instantiation of~$\forall x$ with \mbox{$x=a$}.
%
In a second step, we prove 
\mbox{$\eqref{eq:hcmod2.1} \models \eqref{eq:hcmod4.4} \to \Phi(\mp_{\it c})$}.
\end{proofs}

% \begin{proposition}
% Let $\cI$ be some interpretation satisfying 
% the fact $vertex(a)$
% and the formula~$\eqref{eq:hcmod2.1}$.
% Then,
% $\cI$ is a model of~$\mp_{\it c}$
% iff
% $\cI$ is a model of~$Q_{\it c}$.
% \end{proposition}



==> flattening.tex <==
\section{Verification based on modular programs}
\label{sec:verif}
The ASP semantics is non-monotonic.
%
Thus, in general,
the answer sets of modular program~$\tuple{\cS,\{ (\bp_1 : F_1 ) , \,  (\bp_2 : F_2 ) \}}$
are not necessary the same as the answer sets of~$\tuple{\cS,\{ (\bp_1 \cup \bp_2 : F_1 \wedge F_2 ) \}}$.
%
% the conjunction of modules $\SM_{pred(F)}[F] \wedge \SM_{pred(F')}[F']$ is not equivalent to the whole program $\SM_\vec{p}[F \wedge F']$ for $\vec{p}=pred(F) \cup pred(F')$.
%
In this section, we present conditions under which the answer sets of a modular program coincide with the answer sets of its set of rules where the modular structure of a program is removed (e.g., conditions under which answer sets of the two programs
$\tuple{\cS,\{ (\bp_1 : F_1 ) , \,  (\bp_2 : F_2 ) \}}$
and~$\tuple{\cS,\{ (\bp_1 \cup \bp_2 : F_1 \wedge F_2 ) \}}$ coincide).
%

In the rest of the section, symbol $\mp$ denotes
an arbitrary modular program $\tuple{\cS,\cM}$.
% We say that modular program $\mp$ is \emph{flat} when~$\cM$ is a set of \definitions, that is, there are not nested modular programs in~$\cM$.
The \emph{flattening} of a modular program $P$ is defined as $\flatt{\mp} \eqdef \tuple{\cS,\modules(\mp)}$.
%
For example, $\flatt{\mh^m(E)} = \tuple{\set{\it in},\set{ \eqref{eq:hcmod1.1},\allowbreak \eqref{eq:hcmod2},\allowbreak \eqref{eq:hcmod3},\allowbreak \eqref{eq:hcmod4} ,\allowbreak \eqref{eq:hcmod2.1},\allowbreak \eqref{eq:hcmod2.2},\allowbreak \eqref{eq:pe} }}$,
where we recursively replace each subprogram by its \definitions.


We say that $\mp$ is in $\alpha$-\emph{normal form} (\ANF) if all occurrences of a predicate name in~$\Phi(\mp)$ are free or both they are all bound to a unique occurrence of existential quantifier. For instance, $\mh^m$ is in \ANF{}.
%
Any formula $\Phi(\mp)$ can always be equivalently reduced to $\alpha$-NF by applying so-called $\alpha$-transformations (i.e., choosing new names for quantified variables).
%
In our context, this means changing hidden (auxiliary) predicate names in~$P$ until  \emph{different} symbols are used for distinct auxiliary predicates.
%
Consider, modular program $P'_c$ that differs from $P_c$ in renaming its predicate symbol $r$ by $edge$; and
modular program ${\mh^m}'$ that differs from $\mh^m$ by replacing module $P_c$ by $P'_c$. Program ${\mh^m}'$
 is not in \ANF{}. Yet,  it is 
 equivalent to ${\mh^m}$, since predicate symbol $edge$  is hidden within its submodule $P'_c$.
%
The next theorem states that, when modular program $\mp$ is in \ANF{}, we can ignore its recursive structure and instead consider its flat version.

\begin{comment}
\pedro{We can introduce the definition of \flattable in the proof of the theorem (perhaps as a lemma before, proving its relation to \ANF). But I found it too complicated for the main text.}
\emph{\flattable} if any modular program $\mp' \in \cM$ with $\mp' = \tuple{\cS',\cM'}$ satisfies the following conditions: 
\begin{enumerate}
\item 
predicate symbols occurring both in $\cS$ and $\mp'$ should also occur in $\cS'$,
    \label{item:flattable.2}
\item for any element (\definition or modular program) $M \in \cM$ different from  $\mp'$, 
if a predicate symbol~$p$ occurs in both $\mp'$ and $M$,
then $p \in \cS'$, and
    \label{item:flattable.1}

\item $\mp'$ is \flattable.
\end{enumerate}
\end{comment}

\begin{theorem}\label{thm:flatten}
For any modular program~$\mp$ in \ANF{}, an interpretation  $\cI$ is a model of $\mp$ iff $\cI$ is a model of $\flatt{\mp}$.
\end{theorem}
%
%Note that, in general, not every program is \flattable.
%
%In particular, this is not the case when the same predicate symbol is used locally in two different modules.
%
%Of course, the particular symbol that are used locally are not relevant for the semantics of a modular program.
%
%Hence,we can replace any local predicate symbol by a different predicate symbol and, thus, transform any non-\flattable a program into an equivalent \flattable one.

%{\color{green} YU: sections up to now fully reviewed. Few minor comments left for Jorge;
%Jorge, btw do you remember which problem Pedro suggested to model in addition to HC?
%} 

\red
For our running example,
this theorem affirms  the fact that program~$\mh^m(E)$ is equivalent to flat modular program~$\flatt{\mh^m(E)}$, where we understand the notion of equivalence between modular programs in a natural sense, i.e., modular programs are {\em equivalent} if they coincide on their models.
%

Next, we show  how to relate a flat program with a non-modular program that contains exactly the same rules. We use this result to verify that program in Listing~\ref{list:hamiltonian} satisfies the \hc specification.
\black
To formalize this relation we  focus on a syntax closer to one of logic programs. Consider FO formulas that are conjunctions of rules of the form:
% For HL-modular programs, \cite{har16} showed that there exists such a correspondence between the so called \emph{coherent} HL-modular programs and non-modular programs.
% In the rest of this section, we extend this correspondence to general case of modular programs defined here.
\beq
\ba{r}
\widetilde{\forall} (a_{k+1} \land \dots \land a_l \land \neg a_{l+1} \land \dots 
\land \neg a_m \,\land \neg \neg a_{m+1} \land \dots \land \neg \neg a_n \rar
a_1 
\lor \dots \lor a_k), 
\ea
\eeq{eq:rule_fo}
where all $a_i$ are atoms and $\widetilde{\forall}$ stands for the universal closure of their variables.
%
As usual, the consequent and the antecedent of~\eqref{eq:rule_fo} are  called {\em head} and  {\em body}, respectively.
%
The conjunction $a_{k+1} \land \dots \land a_{l}$ constitutes the {\em positive (part of the) body}.
%
A modular program~$\mp$ is called \emph{simple} if, for every \definition 
$({\bf p} : F) \in \modules(\mp)$, formula~$F$ is a conjunction of rules, and all head predicate symbols in $F$ are intensional (occur in~$\bf p$).
%
This is, in fact, the case of all \definitions we considered so far.
%For the remainder, we study the subclass of simple modular programs that help us connect  logic programs used in practice with a modular framework proposed here.
Let $\intens(\mp)$ collect all intensional predicates in $\mp$, that is $\intens(\mp) \eqdef \bigcup \{ \vec{p} \mid ({\bf p} : F) \in \modules(P)\}$.
%
Then, we form the directed \emph{dependency graph} $DG[\mp]$ by taking $\intens(\mp)$ as nodes and adding an edge $(p,q)$ each time there is a rule occurring in $\mp$ with $p$ in the head and $q$ is in the positive body. 
%
For instance, the dependency graph of program~$\mh^m$ is given in Figure~\ref{fig:example}~(Right).
%
This graph has four strongly connected components, each one consisting of a single node.
In the sequel, we refer to the notion of the dependency graph for a non-modular logic program. A logic program $F$ can be identified with modular program $\tuple{pred(F), \set{(pred(F):F)}}$.

%
A modular program~$\mp$ is 
{\em coherent} if it is simple, in \ANF{}, and satisfies two conditions: 
(i)  every pair of  distinct \definitions
 $({\bf p} : F)$
 and 
$({\bf p'} : F')$  in $\modules(\mp)$ is such that ${\bf p}~\cap~{\bf p'}~=~\emptyset$, 
and (ii)
 for every strongly connected component ${\tt SCC}$ in $DG[\mp]$, 
there is a \definition \hbox{$({\bf p} : F) \in \modules(\mp)$} such that ${\bf p}$ contains 
all vertices in~${\tt SCC}$.
%\end{enumerate}
For example, $\mh^m$ is a coherent program.
%
Now, let us collect the conjunction of all \definition formulas in $\mp$ as
$\formula(P) \eqdef \bigwedge \{F \mid ({\bf p} : F) \in \modules(\mp)\}.$
We can observe, for instance, that $\formula(\mh^m(E)) = \formula(\flatt{\mh^m(E)}) = \fh \wedge \formula(P_e)$, that is, the modular encoding of the \hc problem and the non-modular one share the same rules.
%
We now obtain a similar result to Theorem~3 in~\citep{har16} but
extended to our framework.
%
Together with Proposition~\ref{thm:sm-traditional}, it connects modular programs with logic programs as used in practice.

\red
\begin{theorem}\label{thm:sm-traditional2.hidden}
Let $\mp = \tuple{\cS,\cM}$ be a coherent modular program, $\vec{p}$ be  $\intens(\mp)$, and $\vec{h}$ be $pred(\Phi(\mp))\setminus \cS$.
%
Then, (i) any interpretation~$\cI$ is a model of $\mp$ iff $\cI$ is a model of formula $\exists \bf h$ SM$_\vec{p}[\formula(\mp)]$; (ii)
any  interpretation~$\cI$ is an answer set of $\mp$ iff
 there is some answer set $\cJ$ of~$\formula(\mp)$ such that $\cI=\restr{\cJ}{\cS}$.
\end{theorem}


We use this result to prove that program in Listing~\ref{list:hamiltonian}  satisfies the formal specification~$\mh^m$ of the \hc problem.
%
Therefore, this program also complies with the informal description of this problem as shown in the previous section.
\black

\begin{proposition}
Programs~$\mh^m(E)$ and~$\mh(E)$ have the same answer sets for for any graph $G$ with edges $E$ (mentioning all vertices).
Therefore, the answer sets of (non-modular) program $\fh \wedge \formula(P_e)$ restricted to predicate `$in$' correspond to the Hamiltonian cycles of $G$.
\end{proposition}
\begin{proof}
It can be checked that $\mh^m$ is a coherent program and so it is~$\mh^m(E)$.
Then,
Theorem~\ref{thm:sm-traditional2.hidden} implies that~$\mh^m(E)$ is equivalent 
to~\mbox{$\exists{\bf h} \text{SM}_\vec{p}[\formula(\mh^m) \wedge \formula(P_e)] 
    \!=\! \exists{\bf h} \text{SM}_\vec{p}[\fh \wedge\formula(P_e)]$}
with~${\bf h}=\tuple{vertex,edge,r}$.
%
From Proposition~\ref{thm:sm-traditional},
the models of this last formula are the answer sets of $\fh \wedge F(E)$ restricted to predicate~$in$.
%
Finally
from Proposition~\ref{prop:correct1},
the models of the modular program~$\mh^m(E)$ capture the informal description of the Hamiltonian cycle of~$G$.
\end{proof}

%To continue with our running example, we parameterize the non-modular program $\mh$ with a set of edges~$E$, so that $\mh(E) \eqdef \tuple{\set{\it in},F_{\it halm} \wedge F(E)}$.
%Note that $\mp_c$ as defined above is just the instantiation of %$\mp_c(E)$ with the set of edges of Listing~\ref{list:graph1}.
%
%Then, by Theorems~\ref{thm:sm-traditional} and~\ref{thm:sm-traditional2.hidden}, the answer sets of the logic program~$\mh(E)$ are the same as the answer sets of the modular programs $\mh^m(E)$ and $\flatt{\mh^m(E)}$.
%
%This together with Proposition~\ref{prop:correct1} immediately imply that the non-modular program~$\mh(E)$ correctly computes the \hcs of a graph with edges~$E$.
%
%Note that modular programs $\mh^m(E)$ and~$\flatt{\mh^m(E)}$ are both coherent.

%\begin{corollary}\label{corr:correct1}
%Let $G = \tuple{V,E}$ be some graph with non-empty sets of vertices~$V$ and edges~$E$ where every vertex occurs in some edge and~$\cI$ be some interpretation over the signature~$\set{\mathit{in}}$.
%Then, $\cI$ is an answer set of~$\mh(E)$ iff $\mathit{in}^\cI$ is a \hc of $G$in the sense of Proposition~\ref{prop:correct1}.
%\end{corollary}





\begin{comment}
\newpage


Given a modular program~$\mp=\tuple{\cS,\cM}$,
by $\flatt{\mp} = \tuple{\cS,\cM'}$,
we denote the modular program where $\cM'$ is the set of all \definitions recursively occurring in $\cM$.


\newpage
An 


Our notion of signature is slightly different from the standard in the sense that ``predicate variables'' are included in the signature.

Intuitively, predicates in~$\cP$ represent the shown predicates while predicates in~$\cH$ will be hidden.
Hidden predicates will perform the usual role of second order variables and, thus, we will sometimes refer to them as predicate variables.
We also assume an infinite set of first order \emph{variables}~\mbox{$\cX$}.

------------------------

Let us now extend this definition to cover hidden predicates. 
If ${\bf p}$ and ${\bf h}$ are a pair of tuples of predicate symbols $p_1, \dots, p_n$
and $h_1, \dots, h_m$ with each $p_i \in \cP \cup \cH$ and each $h_i \in \cH$,
and $F$ 
is a formula
then SM$_{\bf p}^{\bf h}[F]$ (called the {\em stable model operator with intensional 
predicates ${\bf p}$ and hidden predicates~${\bf h}$})
denotes the second-order formula 
$$\exists {\bf h} \ \text{SM}_{\bf p}[F],$$
If ${\bf h}$ is the empty tuple, we undertand SM$_{\bf p}^{\bf h}[F]$ as SM$_{\bf p}[F]$.
We will drop the subscript symbol and write just
SM$[F]$ instead of SM$_{\bf p}[F]$, when this does not lead to confusion.


From this point on, we view logic program rules as alternative notation for particular 
types of sentences.  
For example,   we understand the \hc program presented in Section~\ref{sec:trpr} as 
an abbreviation for the sentence SM$_{\bf p}^{\bf h}[F_{\mathit{ham}}]$
where
${\bf p} = \tuple{{\it edge}, {\it vertex}, {\it r}, {\it in} }$,
${\bf h} = \tuple{{\it edge}, {\it vertex}, {\it r} }$
and
 $F_{\mathit{ham}}$ is the conjunction of the following formulas:
% \beq
%  \ba{ll}
% %\begin{align*}
% % &{\it edge}(a, a')\wedge \;\; \dots \;\; \wedge {\it edge}(c, c') \; \\
% &\forall x y({\it edge}(x,y) \rar {\it vertex}(x)) \; \\
% &\forall x y({\it edge}(y,x) \rar {\it vertex}(x)) \; \\
% &\forall x y( (\neg\neg  {\it in}(x,y) \wedge {\it edge}(x,y)) \rar {\it 
% in}(x,y)) \; \\
% &\forall x y z(({\it in}(x,y)\wedge {\it in}(x,z)\wedge \neg(y=z) )\rar\bot) 
% \; \\
% &\forall x y z(({\it in}(x,z)\wedge {\it in}(y,z)\wedge \neg(x=y)) \rar\bot) 
% \; \\
% &\forall x y({\it in}(x,y) \rar {\it r}(x, y)) \; \\
% &\forall x y z(({\it r}(x,z) \wedge {\it r}(z,y))\rar {\it r}(x,y)) \; \\
% &\forall x y ((\neg {\it r}(x, y)\wedge {\it vertex}(x)\wedge {\it 
% vertex}(y))\rar \bot) \\ 
% \ea
% \eeq{eq:hc2}
with $x, y, z$ variables.\footnote{In 
logic programming it is customary to use uppercase letters to denote variables. 
In the literature on logic it is the specific letter used that indicates 
whether a symbol is  an object constant or a variable (with letters drawn from the 
beginning of the alphabet typically used for the former and letters from the end 
of the alphabet for the latter). We utilize both of these traditions 
depending on the context. %whether we use the syntax stemming from logic programming or logic.
}
Note that ${\bf h}$ contains all predicate symbols but $\mathit{in}$,
which is precisely the only predicate symbol for which the directive $\tt\#show$ exists in the program.

\begin{theorem}\label{thm:sm-traditional}
Let $\Pi$ be a logic program over a signature~$\Sigma = \tuple{\cP,\cH,\cC}$
and let $\cI$ be any Herbrand interpretation over~$\Sigma$.
Let also 
$\vec{p}$ be a tuple containing all predicate symbols in $\cP \cup \cH$
and
$\vec{h}$ be a tuple containing all predicate symbols in $\cH$.
Then, the following conditions are equivalent:
 \begin{itemize}
\setlength\itemsep{0em}
\item $\cI$ is a model of SM$_{\bf p}^{\bf h}[\Pi]$,
\item there is a model $\cJ$ of SM$_{\bf p}[\Pi]$ over
$\Sigma' = \tuple{\cP\cup \cH,\emptyset,\cC}$ such that $\restr{\cJ}{\Sigma'} = \cI$,
\item there is an answer set $\cJ$ of $\Pi$ over
$\Sigma' = \tuple{\cP\cup \cH,\emptyset,\cC}$ such that $\restr{\cJ}{\Sigma'} = \cI$,.
\end{itemize}
\end{theorem}
\end{comment}

==> hidden.tex <==
%!TEX root = verification-modular-show.tex
\section{Nested modular programs}\label{sec:modlog}

\red
In the methodology that we propose, the use of modular logic programs as formal specifications is advocated.
%
We depart from the work on modular logic programs by~\citeN{har16}, where each module/logic program of the modular program is a FO formula, whose semantics is captured by the SM operator.
%
This choice is motivated by two factors:
\begin{itemize}[noitemsep]
\item The first-order nature of Harrison and Lierler formalism,
which allows us to argue about the meaning of each module without grounding:
%
to use logic programs as a specification language, 
it is essential that the meaning of its parts can be assessed independently of any particular instance of the problem.
\item The SM operator -- a technical tool for capturing semantics of logic programs -- has been well studied in the literature and manifold technical results (including  theorems on splitting or constraints, for instance) are readily available.
\end{itemize}
%
To adapt this modular approach to the needs of our goal,
we extend it  in two ways:
(i)~handling auxiliary predicates inside modules
% through a formal semantics for the directive {\tt \#show}
and (ii) introducing nested modules.


% We proceed to define now our extension of \cite{har16} that incorporates
% public predicates and nested modules.
%
We start by defining a \emph{\definition} $\cM$ as a pair \mbox{$(\vec{p}:F)$}, where $\vec{p}$ is a tuple of intensional predicate symbols and $F$ is a \mbox{FO formula}.
%
The semantics of a \definition \mbox{$M=\defm{\vec{p}}{F}$} is captured by the formula $\Phi(M) \eqdef \SM_\vec{p}[F]$.
%
When $\vec{p}$ is empty, we write~$F$ in place of \definition \mbox{$(\vec{p}:F)$} --- indeed,  $\Phi(M)$ amounts to $F$.
%
It is easy to see that a logic program~$F$ can be identified with the \definition \mbox{$\defm{pred(F)}{F}$}. % as they have identical answer sets.
%When $F$ is 
%A standard logic program $F$ corresponds to a \definition \mbox{$\defm{pred(F)}{F}$} where all predicate symbols are intensional.
%
The \definition \mbox{$\defm{pred(F)}{F}$} assumes all predicate symbols in $F$ to be intensional.
If we leave some of them as extensional, then their extent is not ``minimized.''
%
For instance, an answer set of rule $\eqref{eq:hce1}$ alone --- \definition $\defm{edge,vertex}{\eqref{eq:hce1}}$ --- is empty; whereas in a \definition~$\defm{vertex}{\eqref{eq:hce1}}$
no assumption is made on extensional predicate $edge$, while $vertex$ would exactly collect all left arguments of $edge$.
%
% For simplicity, in the rest of the paper we will just identify each \definition $M$ with its SO-formula~$\Phi(M)$.

\black

A \emph{modular program} is a pair ${\mp = \tuple{\cS,\cM}}$ where $\cS \subseteq \cP$ is the set of \emph{public (or $\cS$hown)} predicate symbols and $\cM$ is the set of \emph{modules} $\{M_1,\dots,M_n\}$, where $M_i$ ($1\leq i\leq n$) is either a \emph{\definition} or another modular program (called  \emph{subprogram} of $P$), so that all predicate symbols occurring in $\mp$ are in $\cP$.
%
A modular program can be depicted as a hierarchical tree, whose leafs are \definitions.
%
%
The interpretation of a modular program $P=\tuple{\cS, \cM}$ is captured by the (recursively defined) formula:
$$
\Phi(\mp)
	\ \ \eqdef \ \ \exists \vec{h} \
\bigwedge_{M_i \in \cM}
\Phi(M_i),
$$
where $\vec{h}$ contains all free predicate symbols in $\Phi(M_i)$ that are not in $\cS$.
%
Notice that, if~$M_i$ is a \definition $\defm{\vec{p}}{F}$, then $\Phi(M_i)=\SM_\vec{p}[F]$ as we defined before, while if $M_i$ is a subprogram, we apply the formula above recursively.
%It is easy to see that if~$M_i$ is a \definition then all of its predicate symbols are public.
%
We say that an interpretation~$\cI$ is a \emph{model} of a modular program~$\mp$,
when it satisfies the formula~$\Phi(\mp)$.
As in the previous section,
we say that~$\cI$ over the signature~$pred(\Phi(\mp))$ is an \emph{answer set} of a modular program~$\mp$ when it is a Herbrand model of~$\mp$.
Note how $pred(\Phi(\mp))$ coincide with public predicate symbols $\cS$.
%
Under logic programming syntax (like Listing~\ref{list:hamiltonian}), public predicates are declared via {\tt \#show} clauses. % inside the module.
\red
When a modular program has a special form $\tuple{pred(F), \set{(\vec{p}:F)}}$, we identify it with  definition $(\vec{p}:F)$. 

\black
We define $\modules(P)$ as the set of all \definitions in $P$ at any level in the hierarchy.
%
\mbox{Program~$\mp=\tuple{\cS,\cM}$} is said to be \emph{flat} when it does not contain subprograms, i.e., $\cM$ coincides with $\modules(P)$.
%
If ${\mp = \tuple{\cS,\cM}}$ is flat and $\cS$ is the set of all predicate symbols occurring in $\cM$ (i.e. all predicates are public), then $\mp$ is called an \emph{\mbox{HL-modular} program} and corresponds to the definition of modular programs from~\citep{har16}.


We now illustrate a modular program that mimics 
the encoding~$\fh$ (defined in Section~\ref{sec:sm}) of the \hc derived from Listing~\ref{list:hamiltonian}.
% without {\tt \#show} statement. We construct an HL-modular program for this purpose.
We  observe that this modular program comprises the same rules as~$\fh$
and has the same answer sets,
but
%Yet, unlike encoding~\eqref{eq:hc2} that only intuitively groups the rules,
adds explicit structure.
Each of its modules carries its own formal and intuitive meaning. 
The \hc modular program consists of  the following \definitions:
\begin{IEEEeqnarray}{lCCl}
( {\it vertex} & : & \eqref{eq:hce1} \wedge \eqref{eq:hce2} & \ ) \label{eq:hcmod1.1}\\
({\it in} & : & \eqref{eq:choicerulefo}& \ )
\label{eq:hcmod2}\\
({\it r}& : & \eqref{eq:hcr1} \wedge \eqref{eq:hcr2}& \ )
\label{eq:hcmod3}
\end{IEEEeqnarray}
%
%\begin{align}
% &\text{SM}_{{\it edge}}[{\it edge}(a, a')\wedge \;\; \dots \;\; \wedge {\it 
% edge}(c, c') ]\label{eq:hcmod1}\\
%&\begin{aligned}
%\text{SM}_{{\it vertex}}[&\forall x y(  {\it edge}(x,y)  \rar %{\it vertex}(x))\, \wedge\\
%&\forall x y(  {\it edge}(y,x)  \rar {\it vertex}(x))
%]
%\end{aligned}
%\label{eq:hcmod1.1}
%\\
%&\text{SM}_{{\it in}}[\forall x y(\neg \neg {\it in}(x,y) %\wedge {\it edge}(x,y) \rar {\it in}(x,y)]
%\label{eq:hcmod2}
%\\
%&
%\begin{aligned}
%\text{SM}_{{\it r}}[&\forall x y({\it in}(x,y) \rar {\it r}(x, %y)) \,\wedge\\
%\forall x y z({\it r}(x,z) \wedge {\it r}(z,y)\rar {\it %r}(x,y))]
%\end{aligned}
%\label{eq:hcmod3}
%\end{align}
%
together with formulas~\eqref{eq:hcmod4},~\eqref{eq:hcmod2.1}, and~\eqref{eq:hcmod2.2}
that form \definitions, where all predicates are extensional.
%
\red
This presentation is in spirit with the HL-modular program in~\citep{har16} given for the \hc encoding.
Now, observe how predicate symbol~$r$ only occurs in the \definitions~\eqref{eq:hcmod2} and~\eqref{eq:hcmod4}.
%
We can hide this symbol from the rest of the modular program by encapsulating these two \definitions
in the following modular program
$
% \begin{gather}
    \mp_c = \tuple{\, \{ {\it vertex,\, in} \}, \{ \eqref{eq:hcmod3} ,\, \eqref{eq:hcmod4} \}\,}
%     \label{eq:modular.program.connected}
% \end{gather}
.$
This modular program corresponds to rules~4-6 in Listing~\ref{list:hamiltonian}
and intuitively means that the extent of predicate symbol~$in$ forms a strongly connected graph covering all vertices.
%
The only public predicates of modular program $\mp_c$ are~${\it vertex} $ and  ${\it in}$.
We can replace modular program $\mp_c$ by any other modular program 
that ensures the same property on the same  public predicates.
%
%This can be done independently of the auxiliary predicates used in this new module.
For instance, consider \definitions
\begin{align}
&\begin{aligned}
\big( {\it \rap} & : & \forall y\big(\inp(a,y) \rar \rap(y)\big) \,\wedge%\\
%&
\forall x y \big(\inp(x,y) \wedge \rap(x)\rar \rap(y)\big) &  \big)\\
\end{aligned}
% \label{eq:hcmod1.1}
\label{eq:hcmod3.2}
\\
&\forall y \big(\neg {\it ra}(y)\wedge {\it vertex}(y) \rar \bot\big)
\label{eq:hcmod4.2}
\end{align}
and
modular program~$Q_{\it c} = \tuple{\set{\it vertex, in},\set{ \eqref{eq:hcmod3.2},\eqref{eq:hcmod4.2} }}$.
This modular program encapsulates rules in Listing~\ref{list:hamiltonian2}.
Its intuitive meaning coincides with that of modular program~$\mp_c$ (despite their differences in the use of auxiliary predicates).
%:the extent of~$in$ forms a strongly connected graph covering all vertices.
In Section~\ref{sec:eqp} we formally relate these two modular programs, $\mp_c$ and $Q_c$, illustrating their interchangeability.



\section{A formal specification language}
\label{sec:specification}

Modular programs allow us to construct arguments about a correspondence of their modules to their informal meaning in isolation.
%
In this section,
we argue this correspondence for the modular program
\begin{gather}
\mh^m = \tuple{\, \set{\it edge,\, in},\,\set{ \eqref{eq:hcmod1.1}, \eqref{eq:hcmod2},\, \mp_{lc} } \,}
\end{gather}
encoding the \hc problem, where 
$\mp_c = \tuple{\, \{ {\it vertex,\, in} \}, \{ \eqref{eq:hcmod3} ,\, \eqref{eq:hcmod4} \}\,}$
and
$\mp_{lc} = \tuple{\, \{ {\it vertex,\, in} \}, \{ \mp_c ,\, \eqref{eq:hcmod2.1} \}\,}$.
%
% Note that~$\mp_c$ is a nested modular program itself.%
%
We include proof sketches of these arguments to illustrate how this methodology can be used in practice.
\black
%
We first present the informal readings of all \definitions occurring in the program --- i.e., members of  $\modules(\mh^m)$.
The \definitions~\eqref{eq:hcmod1.1}-\eqref{eq:hcmod3} intuitively formulate the following {\em Statements}:
\begin{enumerate} 
\setlength\itemsep{0em}
% \item\label{l:item1}  An Herbrand {\it edge}-stable model of \definition~\eqref{eq:hcmod1} is any  Herbrand 
% interpretation $I$ over $\sigma(\mh)$ such that the extension\footnote{The {\sl extension} of a predicate in an interpretation is the set of 
% tuples that satisfy the predicate in that interpretation.} of the ${\it 
% edge}$ predicate in $I$ corresponds to the  facts in~\eqref{eq:hcfacts} (which encode a given graph). 
\item\label{l:item2}
In any model of~\eqref{eq:hcmod1.1},
the extent of ${\it vertex}$ corresponds to the objects that occur in the extent of ${\it edge}$.

\item\label{l:item3}
In any model of~\eqref{eq:hcmod2},
the extent of ${\it in}$ is a subset of the extent of 
 ${\it edge}$. 
\item\label{l:item5} In any model of~\eqref{eq:hcmod3},
the extent of {\it r} is the transitive closure of the extent of {\it in}.
\end{enumerate}
These statements can be seen as informal achievements of each \definition in the sense of~\cite{lifschitz17a}.
%
Yet, these statements are agnostic to the context where \definitions appear.
%
This closely aligns with good software engineering practices, where the emphasis is made on modularity/independence of code development.
An intuitive meaning of formulas~\eqref{eq:hcmod4},~\eqref{eq:hcmod2.1} and~\eqref{eq:hcmod2.2} is self explanatory given the underlying conventions of FO logic: %and translates into the following informal statements:
\begin{enumerate}
\setcounter{enumi}{3}
\item\label{l:hcmod4} In any model of~\eqref{eq:hcmod4},
the extent of ${\it r}$ contains each possible pair of vertices.
\item\label{l:hcmod2.1} In any model of~\eqref{eq:hcmod2.1},
the extent of ${\it in}$ does not contain two different pairs with the same left component.
\item\label{l:hcmod2.2} In any model of~\eqref{eq:hcmod2.2},
the extent of ${\it in}$ does not contain two different pairs with the same right component.
\end{enumerate}
Statements~\ref{l:item5} and~\ref{l:hcmod4} translate into a joint {\em Statement} about module $\mp_c$:
\begin{enumerate}
\setcounter{enumi}{6}
\item\label{l:hcmod7}
In any model of~$\mp_c$,
the extent of ${\it in}$ forms a strongly connected graph covering all vertices.
\end{enumerate}
\red
This plus Statement~\ref{l:hcmod2.1} lead to the following statement about~$\mp_{lc}$,
\begin{enumerate}
\setcounter{enumi}{7}
\item\label{l:hcmod8a}
In any model of~$\mp_{lc}$,
the extent of ${\it in}$ is a \hc.
\end{enumerate}
\black


Note that each subcomponent of the \hc modular program is small enough so that the verification of respective statements is a manageable and self-isolated task. 
%
In~\cite{cab20}, we use properties of the $\SM$ operator to provide formal proofs for the correctness of these statements.
%
For instance, the following result formalizes Statement~\ref{l:item5}.



\begin{proposition}
\label{prop:transitive.closure}
Let formula $F^{tr}_{qp}$ be 
\beq
\forall xy\big(p(x,y)\rar q(x,y)\big)\,\wedge
\forall xyz\big(q(x,z)\wedge q(z,y)\rar q(x,y)\big)
\eeq{eq:formulatheorem}
For any arbitrary predicates $p$ and $q$, any model $\cI$ of 
${\text{\rm SM}}_{q}[F^{tr}_{qp}]$
is such that the    
the extent of {\it q} is the transitive closure of the relation constructed from the extent of {\it p}.
\end{proposition}
\begin{proofs}
By Remark~1 from \citep{fer09}, we can replace the $\SM_q$ operator in
${\text{\rm SM}}_{q}[F^{tr}_{qp}]$
by $\text{CIRC}_q$.
%
Each model of~$\hbox{CIRC}_{q}[F^{tr}_{qp}]$ is a model of~$F^{tr}_{qp}$ where the extent of~$q$ is minimal. Given FO formula $F^{tr}_{qp}$, this suffices to capture the transitive closure of the extent of~{\it p}.
\end{proofs}

\red
The semantics of \definition~\eqref{eq:hcmod3} is given by the SO formula 
\mbox{$\text{SM}_{{\it r}}[  \eqref{eq:hcr1} \wedge \eqref{eq:hcr2}  ]$}.
%
Proposition~\ref{prop:transitive.closure} proves Statement~\ref{l:item5}: indeed, take $p$ and $q$ to be $\mathit{in}$ and~$\mathit{r}$, respectively.
%
The rest of the modules admit similar proofs that we omit here for space reasons.
%
Obviously, the semantics of a module is given by a SO formula, which at times is complex for providing intuitive arguments about its formulas. Yet, here we are able to construct an intuitive justification 
about  the correspondence of a module and its informal meaning. In this construction, we rely on the relation between minimal models of a FO formula of a module and its formal SO semantics.
%
In other cases, similar arguments 
rely on the relation between the completion~\cite{cla78} of a FO formula of a module and its formal SO semantics.
% (The notion of program's completion was first introduced in.)
%
Note that, given the modular nature of our approach,
the conditions necessary to reduce the SM operator to a simpler formalism are checked in each module rather than on the whole program.
%
In this sense,
we may expect that  modules can often be reduced either to circumscription or completion of FO formulas.
\black


The proposition below states the correctness of Statement~\ref{l:hcmod7} about modular program~$\mp_c$. For an interpretation $\cI$ and predicate symbol $p$, by $p^\cI$ we denote an extent of~$p$ in~$\cI$.  


\begin{proposition}\label{prop:connectivity}
Let $F^{tr}_{qp}$ be formula~\eqref{eq:formulatheorem} and
$F_{v}$ be formula
\beq \forall x y (  \neg{\it q}(x, y) \wedge {\it v}(x)\wedge 
{\it v}(y)\rar \bot).
\eeq{eq:formulatheorem2}
$P_c^{v,p} = \tuple{\set{v,p}, \set{\,(q :F^{tr}_{qp}),\, F_v\,}}$
be a modular program
and
$\tuple{v^{\cI},p^{\cI}}$
be a graph.
%
Then, $\cI$ is a model of~$P_c^{v,p}$
iff 
for every pair \mbox{$a,b \in v^{\cI}$} of distinct vertices,
there is a directed path from~$a$ to~$b$.
\red
Furthermore,
for the modular program~$P_{lc}^{v,p} = \tuple{\set{v,p}, \set{\, P_c^{v,p}, \, \eqref{eq:formulatheorem2b} \,}}$ with
\begin{gather}
\forall x y z({\it p}(x,y)\wedge {\it p}(x,z)\wedge \neg(y=z) \rar\bot) 
    \label{eq:formulatheorem2b}
\end{gather}
we get that
$\cI$ is a model of~$P_{lc}$
iff $p^{\cI}$ are the edges of a Hamiltonian cycle of~$\tuple{v^{\cI},p^{\cI}}$.
%
The opposite direction is easy to check.
\end{proposition}

\begin{proofs}
% The graph is connected iff, for every pair of vertices \mbox{$a,b \in v^{\cI}$},
% there is a directed path from $a$ to $b$.
% , that is, there is a subset $\set{a_0, \dotsc, a_n} \subseteq v^\cI$
% such that $a_0 = a$, $a_n = b$ and every $1 \leq i \leq n$,
% satisfies
% $(a_{i-1},a_{i}) \in p^\cI$.
Note first that \eqref{eq:formulatheorem2} is classically equivalent to  $\forall x y ( {\it v}(x)\wedge {\it v}(y)\rar {\it q}(x, y))$,
so any pair of vertices satisfies $(a,b) \in q^\cI$.
%
From Proposition~\ref{prop:transitive.closure},
relation~$q^\cI$ is the transitive closure of~$p^\cI$.
Hence, such path always exists.

\red
Furthermore,
if $\cI$ is a model of $P_{lc}^{v,p}$,
the above implies
that for any pair \mbox{$v_1,v_m \in v^{\cI}$} of vertices,
there is a directed path
$(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1}, v_m)$
in graph $\tuple{v^{\cI},p^{\cI}}$.
Hence,
there is a directed walk
\beq 
(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1},v_m),\allowbreak (v_{m+1},v_{m+1}),\dotsc,\allowbreak(v_n,v_1)
\eeq{eq:path}
in graph $\tuple{\vertex^{\cI^+},\inp^{\cI}}$
such that  every vertex in $\vertex^{\cI}$ appears in it.
%
Since $\cI$ is also a model of~$\eqref{eq:formulatheorem2b}$, Statements~\ref{l:hcmod2.1} is applicable.
%
This implies $v_i \neq v_j$ for all $i \neq j$
and, thus, that all edges in~\eqref{eq:path} are distinct.
%
Therefore, that~\eqref{eq:path} is a cycle.
%
Since this cycle also covers all vertices of~$\tuple{v^{\cI},p^{\cI}}$,
we get that it is a Hamiltonian cycle.
%
The other direction is easy to verify.
\end{proofs}

\noindent
Modular program $\mp_{lc}$ coincides with modular program
% \mbox{$\tuple{\set{v,p}, \set{\,(q : F^{tr}_{qp}),\, F_v\,}}$}
$\mp_{lc}^{v,p}$
when  predicate symbols~$v$,~$p$ and~$q$ are replaced by~$\mathit{vertex}$, $\mathit{in}$ and~$\mathit{r}$, respectively.
%
It immediately follows that Statement~\ref{l:hcmod8a}  is correct.
%
Note also that~$\mp_c$ also preserves this meaning inside a larger modular program mentioning predicate symbol $r$ in other parts because $r$ in~$\mp_{lc}$ is hidden or \emph{local} (existentially quantified $\Phi(\mp_{lc})$) so that its use elsewhere in larger modular program has a different meaning.
%

To complete the modularization of the \hc problem, we define  the encoding of a graph instance as follows.
%
Given a set $E$ of graph edges, let $\mp_e$ denote a \definition
%we define
\beq
% \begin{aligned}
\big(\, edge :  \bigwedge\set{\mathit{edge}(a,b) \mid (a,b) \in E} \,\big)
%\\
%M(E) \quad &\eqdef \quad \text{\normalfont SM}_{\mathit{edge}}[\mp_e]
% \end{aligned}
\eeq{eq:pe}
% and the \definition $M(E) \eqdef \text{\normalfont SM}_{\mathit{edge}}[\mp_e]$.
%
Then, the \hc problem on a graph with edges~$E$
is encoded by defining modular program~$\mh^m(E) = \tuple{ \, \set{\it in}, \, \set{ \mh^m , \, \mp_e  } \, }$.
The intuitive meaning of \definition  $\mp_e$  culminates in  {\em Statement}:
\begin{enumerate}
\setcounter{enumi}{8}
\item\label{l:hcmod8}
In any model of~$\mp_e$,
the extent of ${\it edge}$ coincides with set $E$ of edges.
\end{enumerate}
We are now ready to state the result that pins the proposed methodology at work.
\red

\begin{proposition}\label{prop:correct1}
Let $G = \tuple{V,E}$ be a graph with non-empty sets of vertices~$V$ and edges~$E$, where every vertex occurs in some edge, and~$\cI$ be an interpretation over the signature~$\set{\mathit{in}}$.
Then,
$\cI$ is an answer set of~$\mh^m(E)$ iff
$\mathit{in}^\cI$ is a \hc of $G$,
 that is,
\begin{enumerate}
    \item $V = \set{ a \mid (a,b) \in \mathit{in}^\cI } \cup \set{ b \mid (a,b) \in \mathit{in}^\cI}$
    
    \item the elements of $\mathit{in}^\cI$ can be arranged as a directed path
    $(v_1,v_2),(v_2,v_3),\dots, (v_n,v_1)$
    so that $v_1,\dotsc,v_n$ are pairwise distinct.
\end{enumerate}
\end{proposition}

The proof is obtained by combining the results corresponding to the submodules of program~$\mh^m(E)$
--- we say submodules here to reflect on the fact that modular programs have recursive structure so that a module of a program may itself consist of modules and so forth.
%
For instance, we formalized
Statement~\ref{l:hcmod8} in Proposition~\ref{prop:connectivity} about submodule $\cP_{lc}$ of program~$\mh^m(E)$.
%
The formalization of other statements is presented at~\cite{cab20}.
%
We take them here for granted.
% We sketch a proof for the left to right direction.
A similar proof at its full length is given at~\cite{cab20}; yet, in that paper HL-modular programs are used to capture the \hc problem which provide no account for {\tt \#show} statements and recursive submodules.
%
The proof presented here is also slightly simplified by the use of recursive modules.

\begin{proofs}
% The proof is obtained by combining the results corresponding to all the modules of program~$\mh^m(E)$, whose informal statements can be found above.
% %
% In particular,
% we have seen how statement~\ref{l:item6} was formalized in Proposition~\ref{prop:connectivity}.
% Note that any model~$\cI$ of \eqref{eq:hcmod1.1}-\eqref{eq:hcmod2}
% satisfies that~$\tuple{\vertex^\cI,\inp^\cI}$ is a subgraph of~$\tuple{\vertex^\cI,\edge^\cI}$
% (statements~\ref{l:item2}-\ref{l:item3}).
% Furthermore,
% from Proposition~\ref{prop:connectivity},
% for any model~$\cI$ of~$\mp_{\it c}$
% and any pair of vertices $v_1,v_n \in \vertex^\cI$,
% there is a directed path
% $(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1}, v_m)$.
% Hence,
% there is a directed path
% $(v_1,v_2),\allowbreak(v_2,v_3),\allowbreak(v_3,v_4),\dots,\allowbreak(v_{m-1},v_m),\allowbreak (v_{m+1},v_{m+1}),\dotsc,\allowbreak(v_n,v_1)$.
% Finally, we can show that this is exactly the extension of  predicate~$\inp$.
% Any model of~$\mp_{\it c}$ that is also a model of~$\eqref{eq:hcmod2.1} \wedge \eqref{eq:hcmod2.2}$ and any vertex $v_i$ with $1 \leq i \leq n$ satisfies that
% $(v_{i-1},v_i)$ and $(v_i,v_{i+1})$,
% with $v_0 = v_{n+1} = v_1$,
% are the only pairs in $\inp^\cI$
% where $v_i$ occurs.
% As a result, we get $\vertex^\cI = \{v_1,\dotsc,v_n\}$
% and $\inp^\cI = \{ (v_1,v_2),\dots,(v_n,v_1) \}$.
% ================
  Take interpretation $\cI$ to be an answer set of~$\mh^m(E)$. It is such that there exists an Herbrand interpretation  
 $\cI^+$ over signature $in,vertex,edge$ so that
 $\cI^+$  coincides with~$\cI$ on the extent of $in$ and is a model of the submodules of $\mh^m(E)$, namely,
  \eqref{eq:hcmod1.1}, \eqref{eq:hcmod2},\, $\mp_{lc}$
 and $\mp_e$.
Thus, interpretation  
 $\cI^+$  adheres to  Statements~1,2,8,9 about these submodules.  
 Since interpretation $\cI^+$ is a Herbrand model of $\mp_e$ it is easy to see how the extent of $edge^{\cI^+}$ coincides with set~$E$ (Statement~\ref{l:hcmod8}).
 Since interpretation $\cI^+$ is a model of \eqref{eq:hcmod1.1}, the extent of $vertex^{\cI^+}$ coincides with set $V$ (Statement~\ref{l:item2}).
 Since interpretation $\cI^+$ is a model of  \eqref{eq:hcmod2},
it follows
 that~$\tuple{\vertex^{\cI^+},\inp^{\cI^+}}$ is a subgraph of~$\tuple{\vertex^{\cI^+},\edge^{\cI^+}}$
(Statement~\ref{l:item3}).
%
Finally, from Proposition~\ref{prop:connectivity}, it follows
$\tuple{\vertex^{\cI^+},\inp^{\cI^+}}$
is a \hc of~$\tuple{\vertex^{\cI^+},\inp^{\cI^+}}$ and, thus, also of~~$\tuple{\vertex^{\cI^+},\edge^{\cI^+}}$.
% % Any model of~$\mp_{\it c}$ that is also a model of~$\eqref{eq:hcmod2.1} \wedge \eqref{eq:hcmod2.2}$ and any vertex $v_i$ with $1 \leq i \leq n$ satisfies that
% % $(v_{i-1},v_i)$ and $(v_i,v_{i+1})$,
% % with $v_0 = v_{n+1} = v_1$,
% % are the only pairs in $\inp^\cI$
% % where $v_i$ occurs.
% % As a result, we get $\vertex^\cI = \{v_1,\dotsc,v_n\}$
% % and $\inp^\cI = \{ (v_1,v_2),\dots,(v_n,v_1) \}$.
% Consequently, this path indeed forms a Hamiltonian cycle of $(V,E)$.
% Furthermore, since the path contains all vertices,
% Statements~\ref{l:hcmod2.1} also imply that path~\eqref{eq:path} contains all tuples in $\inp^{\cI^+}$.
%
% By construction of path~\eqref{eq:path},
% all of its pairs are within $\inp^{\cI^+}$. 
%
Finally,
recall that
$\inp^{\cI^+}=\inp^{\cI}$,
so the result holds.
%  Statements~\ref{l:hcmod2.1} and
% $\eqref{eq:hcmod2.1} \wedge $
The other direction is easy to check.
\end{proofs}

% % \begin{comment}
% \noindent
% We now draw a parallel between the listed statements and the achievements in Listing~\ref{list:hamiltonian}. In this paragraph all references to line numbers point to this listing. 
% We consider the case when 
% the extent of the predicate $\it edge$ is the set of edges of finite digraph~$G$ in which all vertices occur in some edge (lines 1-2). 
% Intuitively, line 4 corresponds to \definition~\eqref{eq:hcmod1.1}.
% Achievement in lines 5-6 coincides with Statement~\ref{l:item2}. 
% Line~8 corresponds to \definition \eqref{eq:hcmod2}.
% For achievement in lines~\mbox{9-10}, we  consider \definitions~\eqref{eq:hcmod1.1} and \eqref{eq:hcmod2} together (note that this is in spirit of ''achievement philosophy'', where achievement statements make claims of written program so far rather than a specific subprogram or a specific rule. In a modular program formalism advocated here we may be more detailed and point at specific rules or group of rules relevant to the claim of achievement.)
% An HL-modular program containing these \definitions satisfies this achievement based on claims in Statements \ref{l:item2} and \ref{l:item3}.
% Lines 12 and~13 
% in 
% Listing~\ref{list:hamiltonian} correspond to \definition~\eqref{eq:hcmod3}.
% Achievement in line 14 coincides with Statement~\ref{l:item5}. 
% For achievement in line 17, we  consider \definitions~\eqref{eq:hcmod3} and~\eqref{eq:hcmod4}. Statements~\ref{l:item5} and~\ref{l:hcmod4} are sufficient to claim this achievement.  
% Lines 21 and 25 correspond to formulas~\ref{eq:hcmod2.1} and~\ref{eq:hcmod2.2}.
% Statement~\ref{l:hcmod2.1} is sufficient to claim a weaker claim than stated in the achievement at lines 22-23, namely, for every vertex $X$ about which $in(X,\cdot)$ relation holds there is at most one vertex $Y$ so that $in(X,Y)$  holds.
% Yet, in presence of \definitions~\eqref{eq:hcmod3} and~\eqref{eq:hcmod4} when we may fall back on additional Statements~\ref{l:item5} and~\ref{l:hcmod4} the achievement in lines 22-23 follows. Similarly, the claim of achievement in lines 26-27 is a consequence of the presence of \definitions~\eqref{eq:hcmod3},~\eqref{eq:hcmod4}, and~\eqref{eq:hcmod2.2} that translate into Statements~\ref{l:item5},~\ref{l:hcmod4} and~\ref{l:hcmod2.2}. 
% Achievement in line 28 is a consequence of the union of all these statements.  Section 6 elaborates on this fact in great detail illustrating how these statements translate into proof of correctness of the \Hamiltonian cycle encoding.
% {\color{blue} YU:  Note how the claim on "every vertex in achievement" makes things less modular.}
% % \end{comment}

% \jcomment{add some comments/sketch about the proof of above result; check the comment stuff}
% The proof of this result is carried on using the the formalization of the above statements corresponding to all its submodules.

This result shows that modular program~$\mh^m$ actually reflects the \emph{informal description} of the \hc problem.
%
Thus,
we can use this modular program as a \emph{formal specification} of the problem.
%
Next,
we use formal specification provided by $\mh^m$ to \emph{verify} the two logic programs for the \hc problem introduced in Section~\ref{sec:motivation}.
\black





% To obtain the behavior of the program in Listing~\ref{list:hamiltonian} with {\tt \#show} statement, consider a modular program
% $\mp_{\it hc} = \tuple{\set{\it in },\set{ \eqref{eq:hcmod1.1}-\eqref{eq:hcmod3},
% \eqref{eq:hcmod4}-\eqref{eq:hcmod2.2} }}$.
% % only contains the symbol~$\it in$.

% We now  go a step further and give extra structure to our modular program by noticing that the predicate symbol~$\it r$ occurs only in the last two modules and it is not shown.
% In this sense, we define a modular program 
% \mbox{$
% \mp_{\it c} = \tuple{\set{\it in, vertex },\set{ \eqref{eq:hcmod3},\eqref{eq:hcmod4} }}
% $}
% that checks the connectivity of a graph.
% Then, we  define an alternative modular program~$\mp_{\it hc}' = \tuple{\set{\it in},\set{ \eqref{eq:hcmod1.1}, \eqref{eq:hcmod2}, \eqref{eq:hcmod2.1}, \eqref{eq:hcmod2.2}, \, \mp_{\it c} }}$ for the \hc problem.
% This second representation makes explicit that 
% $\mp_{\it c}$ only communicates with the rest of the program through predicate symbols
% $\set{\it in, vertex }$.
% In other words,  predicate symbol $\it r$ is local to 
% $\mp_{\it c}$.
% We can verbalize the  intuitive meaning of the modular program $\mp_{\it c}$ as follows:
% \begin{enumerate}
% \setcounter{enumi}{6}
% \setlength\itemsep{0em}
% \item\label{l:item6} Any model of $\mp_{\it c}$ represents a connected graph, where the relations $\it vertex$ and $\it in$ stand for its sets of vertices and edges, respectively.
% \end{enumerate}
% % Another interesting observation is to view \definitions~\eqref{eq:hcmod1.1} and~\eqref{eq:hcmod2} as a part of the following   modular program $\mp_s= \tuple{\cS_{\it s},\cM_{\it s}}$,
% % where $\cS_{\it s}=\set{edge,vertex,in}$ and
% % $\cM_{\it s} = \set{\eqref{eq:hcmod1.1} -\eqref{eq:hcmod2}}$.  
% % We can verbalise the following intuitive meaning of the modular program $\mp_{\it s}$:
% % \begin{enumerate} [ start=7 ]
% % \setlength\itemsep{0em}
% % \item\label{l:item7} Consider the graph, whose edges and vertexes are encoded by the extents of predicates $edge$ and $vertex$ respectively. 
% % Any model of $\mp_{\it s}$ is such that 
% % the extent of the predicate $in$ corresponds to a subgraph  of 
% % where the relations $\it vertex$ and $\it in$ stand for its sets of vertices and edges, respectively.
% % \end{enumerate}
% % whose show predicates are $in,vertex,edge$ and 

% We introduced two distinct modular programs that differ in the way they define and group their modules. Yet, they represent solutions to the same problem.
% In the next subsection, we show that these two programs indeed have the same models.
% We also connect the practice of modular programs to traditional logic programs.







==> introduction.tex <==
%!TEX root = verification-modular-show.tex

\begin{comment}
Yulia's Notes to address in next revision:

Section 2 last paragraph:
*  Capturing auxiliary predicates as existential quantifiers also formalizes the property that allows us to rename a hidden predicate by a new fresh predicate symbol.

Section 3 first paragraph
* If we leave some of them as extensional, no assumption is made on their extent.

Section 4 the beginning of the second paragraph
*if all occurrences of a predicate name in Φ(P) are free or both they are all bound to a unique occurrence of existential quantifier.
*they are strongly equivalent under the empty context ∅. 

Is top the same as empty context?

\end{comment}
\section{Introduction}

Achieving trustworthy AI systems requires, among other qualities,
the assessment that those systems produce correct judgments\footnote{\emph{Ethics Guidelines For Trustworthy AI}, High-level Expert Group on Artificial Intelligence set up by the European Commission.
%See also \emph{The National Artificial Intelligence Research And Development
%strategic Plan: 2019 Update}, Select Committee On Artificial Intelligence of the National Science \& Technology Council.
} or, in other words, the ability to  verify that produced results adhere to specifications on expected solutions. 
%
These specifications may have the form of expressions in some formal language or may  amount to statements in natural language (consider English used in mathematical texts).
%
Under this trust-oriented perspective, AI systems built upon some Knowledge Representation (KR) paradigm start from an advantageous position, since their behavior is  captured by some declarative machine-interpretable formal language.
%
Moreover, depending on its degree of declarativity, a KR formalism can also be seen as a specification language by itself.
%
%However, sometimes modern KR languages use  elaborate constructs 
%whose correspondence with natural language specifications is not always straightforward.

Answer Set Programming~(ASP)~\cite{niemela99a,martru99a}
is a well-established declarative KR paradigm for solving knowledge-intensive search/optimization problems.
%
Based on logic programming under the \emph{answer set semantics}~\cite{gellif88b},
%,gellif91a}, 
the ASP methodology relies on devising a logic program so that its answer sets are in one-to-one correspondence to the solutions of the target problem.
%
This approach is fully declarative, since the logic program only describes a problem and conditions on its solutions, but abstracts out the way to obtain them, delegated to systems called answer set solvers.
%a call to some ASP solver~\cite{liemar04a,dlv03a,geb07}.
%
%ASP is a specification language itself, but when is an encoding correct? does it correspond to an informal meaning? do different encodings represent the same problem? we normally use different constructs and/or auxiliary predicates
%
Thus, it would seem natural to consider
an ASP program to serve a role of a formal specification on its expected solutions.
%
%An ideal ASP encoding of a problem for this purpose is the one closest to its informal specification.
%
However, %despite its declarative nature, 
the non-monotonicity of the ASP semantics makes it difficult to directly associate an independent meaning to an arbitrary program fragment (as we customary do, for instance, with theories in classical logic).
%
This complicates assessing that a given logic program reflects, in fact, its intended \emph{informal description}.
%
And yet, ASP practitioners do build logic programs in groups of rules and identify each group with some part of the informal specification~\cite{erdo04,lifschitz17a}.
%
Moreover, modifications on a program frequently take place within a group of rules rather than in the program as a whole.
%
The safety of these local modifications normally relies on such properties in ASP  as \emph{splitting}~\cite{liftur94a,felelipa09}.
% or \emph{(ground) modules}~\cite{oikjan06a}.
%--- that can be applied under certain syntactic restrictions.
%

%To overcome this limitation,
With these observations at hand, 
\red
in~\cite{cab20} we proposed a \emph{verification methodology for logic programs} where the argument of correctness of a program is decomposed into respective statements of its parts, relying to this aim on a modular view of ASP~\cite{OikarinenJ09,har16}.
%
In this methodology, a \emph{formal specification} $\Pi$ is formed by a set of modules called \emph{modular program}, so that each module (a set of program rules) is {\em ideally small enough to be naturally related to its informal description} in isolation.
%
This relation can be established using quasi-formal English statements~\cite{den12,lifschitz17a} or relying on classical logic~\cite{lifschitz18a}.
%
The same specification $\Pi$ may serve to describe different (non-modular) ASP programs encoding the same problem, being each encoding $P$ written under a given priority (involving efficiency, readability, flexibility, etc).
%
As usual in \emph{Formal Methods}~\cite{mon03}, \emph{verification} then consists in obtaining a \emph{formal proof} of the correspondence between the verified object (in our case, the non-modular encoding $P$) and its specification (the set $\Pi$ of modules matching the informal aspects of that problem).
%
The example presented in~\cite{cab20}, for instance, proved the correctness of a non-ground ASP program $P$ encoding the Hamiltonian Cycle problem with respect to a specification $\Pi$ consisting of modules as defined in~\cite{har16}.
%
It is important to note that the formal language used in that proof was subject to two important requirements: (i) dealing with stable models of non-ground programs; and (ii) capturing those stable models as an expression that can be formally manipulated.
%
For (i), we could have simply used \emph{Quantified Equilibrium Logic}~\cite{peaval06a} but for (ii) the equivalent formulation in~\cite{ferraris11a} is more suitable, as it captures stable models of a program as a second-order formula\footnote{The need for second-order logic is not surprising: unlike first-order classical logic, the stable models of a first-order program allow capturing a transitive closure relation.}, the SM operator.

The approach in~\cite{cab20}, however, showed some important limitations for \emph{reusing} the obtained proof in a modular way.
%
Once a modular specification is guaranteed, one would expect that the replacement of a module by a different encoding could be reduced to some kind of equivalence between modules without affecting to the rest of the correctness proof.
%
Similarly, one could easily imagine that the whole ASP specification $\Pi$ of some problem (like the Hamiltonian Cycle) could describe, in its turn, a module for a larger program and, again, one would expect that the correctness proof should be reused in some way.
%
The problem here appears when \emph{auxiliary predicates} are involved.
%
These predicates are quite common to improve the solver performance in a given encoding $P$ but, more importantly, they are sometimes indispensable in the specification $\Pi$ to express some property that the ASP language cannot directly capture otherwise~\cite{goncalves16a}. 
%
In both cases, their presence must be removed when proving correctness which, in its turn, normally depends on their \emph{local use in some part of the program}.
%

In this paper, we extend the modular language from~\cite{har16} so that a specification $\Pi$ consists now of a \emph{hierarchical tree} of modules and submodules, each of them possibly declaring its own set of public and hidden predicates at different levels.
%
% This is an important implicit assumption handled during the development cycle that is not formally stated in the program code.
%Our specification language allows declaring public predicates in a module using {\tt \#show} statements (that receive, in this way, a formal treatment), being the rest of predicates considered auxiliary.
%
To illustrate this extension, we revisit the formal proof in~\cite{cab20} for the Hamiltonian Cycle encoding but providing now a hierarchical specification.
%
We also provide an example of module replacement that is verified through an equivalence proof that disregards the existing auxiliary predicates.

\black

The paper starts by providing a running example of this work. % used for illustration and motivation purposes. 
 In Section~\ref{sec:sm}, we revisit the SM operator and extend it with hidden predicates.
% %
 Section~\ref{sec:modlog} presents our modular logic programs.
 Sections~\ref{sec:specification} and~\ref{sec:verif} explain the use of modular programs for formal verification illustrating the proposed methodology on the running example.
% Section~\ref{sec:eqp} studies formal properties of modular programs related to equivalent substitutions of its subparts.
% %
% Section~\ref{sec:conc} concludes the paper.


\section{Motivating example}\label{sec:motivation}


We consider %illustrate the key ideas behind our methodology using 
a well-known domain in the ASP literature: the search of Hamiltonian cycles in a graph.
%
A \hc is a cyclic path from a directed graph that visits each of the graph's vertex exactly once.
%
\begin{figure}[t]
\centering
\begin{tabular}{cc}
%\tiny
\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]
\node[place] (a) {{\it a}};
\node[place] (b)  [right of=a] {{\it b}};
\node[place] (c) [below  of=b] {{\it c}};
\node[place] (d) [below  of=a] {{\it d}};
% (r) edge [loop above] node {} ()
\draw [->,double distance=2pt] (a) to  (b);
\draw [->,double distance=2pt] (b) to  (c);
\draw [->,double distance=2pt] (d) to  (a);
\draw [->,double distance=2pt] (c) to [out=155,in=25] (d);
\draw [->] (d) to [out=-25,in=205] (c);
\end{tikzpicture}
&\hspace{80pt}
\begin{tikzpicture}[shorten >=2pt, auto,scale=0.5, every node/.style={scale=0.5}]
\node[place] (e) {{\it edge}};
\node[place] (v)  [right of=e] {{\it vertex}};
\node[place] (i) [below  of=e] {$\;\;${\it in}$\;\;$ };
\node[place] (r) [below  of=v] {$\;\;\;${\it r}$\;\;$ };
\path[->]
% (r) edge [loop above] node {} ()
(v)   edge[->] node[above] {} (e)
(r)   edge[->] node[above] {} (i)
(i) edge[->] node[below] {} (e)
(r) edge [loop above] node {} ();
\end{tikzpicture}
\end{tabular}
%\normalsize
\caption{Left: graph $G_1$; Right: dependency graph for $\mh^m$.} 
\label{fig:example}
\end{figure}
%
For instance, Figure~\ref{fig:example}~(Left) depicts graph~$G_1$ whose unique Hamiltonian cycle is marked in double lines, whereas Listing~\ref{list:hamiltonian} presents a possible encoding of the problem in the language of ASP solver {\sc clingo}~\citep{geb07}.
% \begin{figure}[ht]

\lstinputlisting[
  caption = {Encoding of a Hamiltonian cycle problem using {\sc clingo}. 
%   The program is annotated with \emph{achievements}.
},
  label={list:hamiltonian},
  basicstyle=\ttfamily\small,
  numbers=left,
  stepnumber=2,
]{lp/hamiltonian.tex}
%
% \end{figure}
% This program is annotated with \emph{achievements}
% following the methodology introduced by~\cite{DBLP:journals/tplp/Lifschitz17}, where he assumes that {\em 
%  ``the programmer would include a comment that states what has been {\em achieved} so far, in a
% certain precise sense.''}
% The properties stated by these achievements are expected to be maintained until the program is
% completed.
The {\tt \#show} directive is used to tell {\sc clingo} which predicates should appear in the obtained answer sets (we call such predicates {\em public}): here only predicate {\tt in/2} -- containing the edges that form the solution -- is declared public. 
%
\lstinputlisting[
  caption = {Facts describing graph $G_1$.
%   The program is annotated with \emph{achievements}.
  },
  label={list:graph1},
  basicstyle=\ttfamily\small
]{lp/graph1.tex}
Now, if we add the facts corresponding to graph $G_1$ depicted in Listing~\ref{list:graph1} and instruct {\sc clingo} to find all the answer sets we obtain the unique Hamiltonian cycle in the graph:
\lstinputlisting[
caption = {Output by {\sc clingo} for program composed of lines in Listing~\ref{list:hamiltonian} and~\ref{list:graph1}.},
label={list:answer},
  basicstyle=\ttfamily\small
]{lp/answer1.tex}

The usual intuitive reading for Listing~\ref{list:hamiltonian} assumes
an informal division of a program
into groups of rules.
%
The ASP practitioners say Rule~3 generates all possible subsets of edges, while Rules~\mbox{7-8} guarantee that connections among them are linear.
%
Rules~\mbox{4-5} are meant to define the auxiliary predicate~$\mathit{r}$ (for ``reachable'') as the transitive closure of predicate~$\mathit{in}$.
%
To assign this meaning to~$r$, we \emph{implicitly assume} that this predicate does not occur  in other rule heads in the rest of the program.
%
Predicate $r$ is then used in  rule~6 to enforce that any pair of vertices are connected.
%
Rules~\mbox{4-6} together guarantee that facts for $in$ form a strongly connected graph covering all vertices in the given graph.

The methodology we propose consists in~(i) making this informal division formal, 
(ii)~arguing that each of these fragments is actually a formalization of the informal claims made, and 
(iii) using these claims to compose an argument about the whole specification.

\red
Sections~\ref{sec:specification} and~\ref{sec:verif} will illustrate the use of this methodology on the running example.
%
We will start by defining a modular specification $\mphs$ 

We start introducing a modular program $\Pi$ that consists of all rules in the encoding Listing~\ref{list:hamiltonian} except the last one. 
This is a somewhat singular case,
in which logic program of interest contains almost exactly the same rules as its modular formal specification.
%and it is the straightforward implementation of the specification.
%
Considered logic program may need to be modified for performance reasons.
%
Usually,
the program development involves a sequence of \emph{refactoring} -- in software engineering, refactoring means improving software attributes without changing its functional external behavior -- iterations, where each new version implies a better performance of the answer set solver, but its correspondence with the original encoding of the problem becomes more and more obscure~\cite{bud15}. In this sense,
\emph{verifying} an ASP program can mean establishing some kind of \emph{equivalence} result between its formal specification in the form of an original ASP program and the final program obtained from the refactoring process~\cite{lier19}.
Continuing with our running example,
 program in Listing~\ref{list:hamiltonian}
produces an excessively large ground program when  utilized on graphs of non trivial size.
\black
It turns out that it is enough to require that all vertices are reachable from some fixed node in the graph (for instance, $a$), provided that rules such as~\mbox{7} and~\mbox{8} restrict all paths to be linear.
%
Rules~\mbox{4-6} of   Listing~\ref{list:hamiltonian} are usually replaced by rules below:
% \begin{figure}[ht]
\lstinputlisting[
  caption = {Alternative code to lines~\mbox{4-6} in Listing~\ref{list:hamiltonian}~\protect\cite{martru99a}.
%   The program is annotated with \emph{achievements}.
},
  label={list:hamiltonian2},
  basicstyle=\ttfamily\small,
  stepnumber=2,
]{lp/hamiltonian2.tex}
% \end{figure}
%
%Since this is an extensively studied example, we know at this point that,
For any input graph with a vertex named~$a$, the answer sets with respect to the public predicate $in$ of both versions of the program are identical. In the paper, we illustrate how our proposed modular framework and advocated methodology accounts for a formal proof that both encodings  are ``essentially'' equivalent and correct.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\color{blue} YU: It does not look like we would have enough space for this aspect within IJCAI paper, so it is dropped for now.}

Listing~\ref{list:hamiltonian} provides an intuitive encoding of the \hc problem in ASP. In practice, it is common that lines 12-16 are replaced by the code presented in Listing~\ref{list:hamiltonian2}~\citep{mar99}.
System {\sc clingo} finds the same solution shown in Listing~\ref{list:answer1} for the modified program. 
This modification deserves some comments:
\begin{enumerate}
\item The modified encoding assumes that there is a vertex named ``$a$'' in the input graph.

\item If to remove the $\tt\#show$ directive in both programs, their answer sets will differ. Yet, these answer sets still represent the same \hcs.

\item The achievements in lines 14 and 14b are different. Yet, they allow us to prove the same achievement in line 17.
\end{enumerate}

{
\lstset{ 
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  firstnumber=12
}
\renewcommand*\thelstnumber{\oldstylenums{\the\value{lstnumber}}b}
\lstinputlisting[
  caption = {Alternative encoding of strong connectivity in a Hamiltonian cycle problem.},
  label={list:hamiltonian2}
]{lp/hamiltonian2.tex}
}

\begin{itemize}
    \item {\color{blue} this is probably a place to present the outline of the paper and speak of its main contributions using the motivation example above. The paragraph below would be one of these. } 
\end{itemize}
In Section~\ref{sec:hamiltonian}, we turn achievements into formal statements, prove their correctness,
and show how one can ensure that they are maintained until the program is
completed. These results, for instance, allow us to illustrate
 that if condition~$1$ holds for the considered \hc encoding in  Listing~\ref{list:hamiltonian} then
replacing rules 12-16 by 12b-16b results in an ''\emph{equivalent}'' program.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
An interesting approach followed by some authors~\cite{den12,har16} consisted in defining an alternative semantics for ASP programs as a collection of \emph{(first-order) program modules} and providing guidelines on how to obtain the informal meaning of each module.
%
This forms a solid starting point for our endeavor, but still lacks for  a proper treatment of auxiliary predicates.
%
%For instance, if we see Rule~2 as a module generating subsets of edges, we can replace it by the classical encoding
%
%\lstinputlisting[
%  basicstyle=\ttfamily\small
%]{lp/negloop.tex}
%where predicate $out$ is local to this pair of rules and should be declared irrelevant for their informal meaning.
%
Once we consider auxiliary predicates,
the lack for a module hierarchy also becomes a limitation: think, for instance, that Listing~\ref{list:hamiltonian} as a whole could become in its turn a module inside a larger program whose correctness proof should obviously reuse the correctness of the Hamiltonian cycle module.

\color{darkred}
%
Therefore, \emph{verifying} an ASP program means establishing a correspondence to another specification language such as, for instance, quasi-formal English statements~\cite{den12,lifschitz17a} or classical logic~\cite{lifschitz18a}.

---------------------


We illustrate this methodology using the Hamiltonian cycle problem as our running example.
%
A modular version of the program in Listing~\ref{list:hamiltonian} is used
as a formal specification of the problem.
%
We reason that the relation between the formal specification of each module and its informal meaning can be easily assessed.
%
The specifications of all modules can be combined to assess that it adheres to the Hamiltonian cycle problem.
%
Finally,
we can prove that the relevant and yet different encoding used by~\cite{martru99a} is correct with respect to this specification.



-------------------------


An additional obstacle that 


-------------------------------
\color{black}

% In this paper, we extend the modular ASP framework from~\cite{har16} in two ways:
% (i) handling auxiliary predicates inside modules through a formal semantics for the directive {\tt \#show} and (ii) introducing nested modules.
% %
% Modules are configured as program fragments satisfying some syntactic conditions and their semantics is defined in terms of the SM operator~\cite{fer09}, a second-order formulation of the answer sets of a first-order theory.
% %
% In this setting, we characterize auxiliary predicates as new existential second-order variables.
% %
% An important advantage of this approach with respect to other modular frameworks like~\cite{oikjan06a} is that it allows proving correctness of modules directly in a first-order representation, so the method does not depend on the program grounding.
% %
% %Using our running example, we illustrate how these features help us arguing the program correctness.
% %














Proving correctness of an ASP program without considering its iterative construction process may become difficult.
%
The first issue is due to the non-modularity of the ASP semantics.

\end{comment}

==> lp/hamiltonian-achievements.tex <==
% input: the set edge/2 of edges of a finite 
% digraph G whose vertices occur in some edge

vertex(X):- edge(X,Y). vertex(X):- edge(Y,X).
% achieved: Set vertex/1 consists of all 
% vertices of the graph G.

{ in(X,Y) }:- edge(X,Y).
% achieved: Set in/2 is the set of edges of 
% some subgraph of G.

r(X,Y):- in(X,Y).  
r(X,Y):- r(X,Z), r(Z,Y).
% achieved: r/2 is transitive closure of in/2

:- not r(X,Y), vertex(X), vertex(Y).
% achieved: Set in/2 is the set of edges of 
% some strongly connected subgraph of G that 
% contains all its vertices

:- in(X,Y), in(X,Z), Y != Z.
% achieved: for every vertex X of G there is 
% at most one vertex Y such that in(X,Y).

:- in(X,Y), in(Z,Y), X != Y.
% achieved: for every vertex Y of G there is 
% at most one vertex X such that in(X,Y)
% achieved: Set in/2 is a Ham-n Cycle of G

#show in/2.
% ach-d: an answer set contains only set in/2
% ach-d: an answer set is a Ham-n Cycle of G


==> lp/hamiltonian2-achievements.tex <==
r(a).
r(Y) :- in(X,Y), r(X).
% achieved: r/1 forms the set of vertices 
% reachable from a in G
:- not r(X), vertex(X).

==> lp/negloop.tex <==
in(X,Y)  :- edge(X,Y), not out(X,Y).
out(X,Y) :- edge(X,Y), not in(X,Y).

==> prop_ham_equivalence.tex <==
\begin{proof}
The proof consists on two steps.
The first shows that
$\vertex(a) \models \Phi(\mp_{\it c}') \leftrightarrow F$
with
\mbox{$F = \exists r\, (\eqref{eq:hcmod3} \wedge \eqref{eq:hcmod4.4})$}
and
\begin{align}
&\forall y (\vertex(a)\wedge\vertex(y)  \rar \rp(a,y))
\label{eq:hcmod4.4}
\end{align}
Furthermore,
$\models \Phi(\mp_{\it c}) \to F$
follows by instantiating $\forall x$ with~$a$.
Then,
the second step consists in showing that
$\eqref{eq:hcmod2.1} \models F \to \Phi(\mp_{\it c})$.
\\[10pt]
For the first step note that~\eqref{eq:hcmod3}
is equivalent to the following formulas
\begin{align}
&\begin{aligned}
\text{CIRC}_{\rp}[&\forall xy(\inp(x,y) \rar \rp(x,y)) \,\wedge\\
&\forall x yz (\rp(x,z) \wedge \rp(z,y)\rar \rp(x,y))]
\end{aligned}
\label{eq:hcmod3.circ.b}
\\
&\begin{aligned}
\text{CIRC}_{\rp}[&\forall xy(\inp(x,y) \rar \rp(x,y)) \,\wedge\\
&\forall x yz (\rp(x,z) \wedge \inp(z,y)\rar \rp(x,y))]
\end{aligned}
\label{eq:hcmod3.circ}
\end{align}
and~\eqref{eq:hcmod3.2} is equivalent to
\begin{align}
&\begin{aligned}
\text{CIRC}_{\rap}[&\forall y(\inp(a,y) \rar \rap(y)) \,\wedge\\
&\forall  yz (\rap(z) \wedge \inp(z,y)\rar \rap(y))]
\end{aligned}
\label{eq:hcmod3.2.circ}
\end{align}
We also can see that
$\forall y (\rp(a,y) \leftrightarrow \rap(y))
\models 
\eqref{eq:hcmod3.circ} \leftrightarrow
\eqref{eq:hcmod3.2.circ}$
and, thus, that~$\Phi(\mp_{\it c}')$ is equivalent to the following formulas
\begin{align}
    &\exists \rp\exists\rap\, 
    (
    \eqref{eq:hcmod3.2.circ}
    \wedge 
    \eqref{eq:hcmod4.2}
    )
    \nonumber
\\
&\exists \rp\exists\rap\, 
    (
    \eqref{eq:hcmod3.2.circ}
    \wedge 
    \eqref{eq:hcmod4.2}
    \wedge (\forall y (\rp(a,y) \leftrightarrow \rap(y)))
    )
    \nonumber
\\
    &\exists \rp\exists\rap\, 
    (
    \eqref{eq:hcmod3.circ}
    \wedge 
    \eqref{eq:hcmod4.2}
    \wedge (\forall y (\rp(a,y) \leftrightarrow \rap(y)))
    )
   \nonumber
\\
    &\exists \rp\exists\rap\, 
    (
    \eqref{eq:hcmod3}
    \wedge 
    \eqref{eq:hcmod4.2}
    \wedge (\forall y (\rp(a,y) \leftrightarrow \rap(y)))
    )
    \label{eq:1:prop:ham.equivalence}
\end{align}
Furthermore,
we also can see that
$\vertex(a) \models \eqref{eq:hcmod4.2} \leftrightarrow 
\eqref{eq:2:prop:ham.equivalence}$
and, thus, that
$\vertex(a) \models \eqref{eq:hcmod4.4} \leftrightarrow 
\eqref{eq:2:prop:ham.equivalence}$
with
\begin{align}
    &\exists \rp\exists\rap\, 
    (
    \eqref{eq:hcmod3}
    \wedge 
    \eqref{eq:hcmod4.4}
    \wedge (\forall y (\rp(a,y) \leftrightarrow \rap(y)))
    )
    \label{eq:2:prop:ham.equivalence}
\end{align}
Then, since the predicate symbol~$\rap$ does not occur neither in~$\eqref{eq:hcmod3.circ}$ nor in~$\eqref{eq:hcmod4.4}$,
we get that
$\models \eqref{eq:2:prop:ham.equivalence} \leftrightarrow F$.
Consequently,
$\vertex(a) \models \Phi(\mp_{\it c}') \leftrightarrow F$
follows.
\\[10pt]
For the second step,
we show
$\eqref{eq:hcmod2.1} \models 
\eqref{eq:hcmod3.circ.b} \wedge \eqref{eq:hcmod4.4} \to  \eqref{eq:hcmod4}$.
Let~$\cI$ be a model of~$\eqref{eq:hcmod2.1} \wedge \eqref{eq:hcmod3.circ.b} \wedge \eqref{eq:hcmod4.4}$.
Note that~\eqref{eq:hcmod4.4}
ensures that~$(a,b) \in \rp^\cI$ for any~$b \in \vertex^\cI$
and thus that, if $(c,a) \in \rp^\cI$ holds,
then~\eqref{eq:hcmod3.circ.b}
ensures that $(c,b) \in \rp^\cI$ also holds.
Hence,
it is enough to show that
$(c,a)\in \rp^\cI$ holds
for any~$c$ such that $c \in \vertex^\cI$.
Furthermore,
\eqref{eq:hcmod4.4}
implies that
$(a,a)\in \rp^\cI$ and $(a,c) \in \rp^\cI$ hold,
and, thus,
$\eqref{eq:hcmod3.circ.b}$
implies that there are paths
\begin{align*}
\set{ (v_0,v_1),(v_1,v_2),...,(v_{n-1},v_{n})} &\subseteq \inp^\cI
\\
\set{ (v_0',v_1'),(v_1',v_2'),...,(v_{m-1}',v_{m}')} &\subseteq \inp^\cI
\end{align*}
with
$v_0 = v_0' = v_n = a$,
$v_m' = c$
and
$v_i \neq v_j$ for $i \neq j$.
Note that, since $\cI$ is a model of~\eqref{eq:hcmod2.1},
we get that $v_i = v_i'$ for all $1 \leq i \leq k$ with $k = \min\set{n,m}$.
Note that $n = m$ implies that $a= v_n = v_m' = c$ and, thus, $(a,c) \in \rp^\cI$.
If $k = m < n$,
the
$v_m = c$
and $(c,a) \in \rp^\cI$.
Otherwise,
we have $k = n < m$ and
$v_n' = a$.
This implies that
$v_{n+1}' = v_1'$
which is a contradiction.
Hence, it must be that
$(a,c) \in \rp^\cI$.
\end{proof}

==> removedpart.tex <==


\section{Logic Programs with {\tt\#show} Statements}

As shown in the previous section,
we can formalise the semantics of logic programs without
$\tt\#show$
directives using the SM operator.
We now formalise the use of this directive.

Given a signature~$\cP$,
a \emph{program} is a pair $\tuple{\cS,F}$,
where $\cS \subseteq \cP$ is a set of predicate symbols
and~$F$ is a FO-formula over~$\cP$.
An interpretation~$\cI$ over~$\cS$
is  an {\em answer set} of~$\tuple{\cS,F}$,
when there is some answer set~$\cJ$ of $F$ over~$\cP$
such that
\mbox{$\restr{\cJ}{\cS} = \cI$},
where by $\restr{\cJ}{\cS}$
we denote an
an interpretation over~$\cS$
that agrees with $\cJ$ in the interpretation of all symbols in $\cS$.

Continuing now with our running example,
it is easy to see that the program obtained by joining Listings~\ref{list:hamiltonian}
and~\ref{list:graph1}
corresponds to the program $\tuple{\set{ \it in },\fh \wedge F_{\it graph}}$.
This program has a unique answer set which only contains the predicate symbol $\it in$.
The extension of this predicate in this answer set is given in
Section~\ref{sec:motivation}.
% Listing~\ref{list:answer1}.

Thanks to the second order nature of the SM operator,
incorporating {\tt\#show} directives amounts to add existential quantifiers for all non-shown predicates.
Formally,
we associate every program $\tuple{\cS,F}$ over signature~$\cP$
with
the second order formula
\begin{gather}
\exists {\bf h} \ \text{SM}_{\bf p}[F],
    \label{eq:sm.hidden}
\end{gather}
over signature $\cS$
where 
$\vec{p}$ is a tuple containing all symbols in~$\cP$ and
${\bf h}$ is a tuple containing all predicate symbols in~$\cP \setminus \cS$.
Note that we assume without loss of generality that every symbol in
\mbox{$\cP \setminus \cS$} is a second order variable.
This implies that
some predicate symbols of the program~$\tuple{\cS,F}$
become second order variables in the formula~\eqref{eq:sm.hidden}.
We call the symbols in $\bf h$ \emph{hidden predicates}.

\begin{theorem}\label{thm:sm-traditional}
Let $\tuple{\cS,F}$ be a program over a signature~$\cP$
and let $\cI$ be any Herbrand interpretation over~$\cS$.
Let also 
$\vec{p}$ be a tuple containing all predicate symbols in $\cP$
and
$\vec{h}$ be a tuple containing all predicate symbols in $\cP \setminus \cS$.
Then, the following conditions are equivalent:
 \begin{itemize}
\setlength\itemsep{0em}
\item $\cI$ is an answer set of $\tuple{\cS,F}$,

\item $\cI$ is a model of $\exists \bf h$ SM$_{\bf p}[F]$.
\end{itemize}
\end{theorem}

\noindent
In our running example,
${\bf h}$ stands for a tuple containing all predicates occurring in the formula~$\fh$, but predicate~$\it in$.
%
If $\vec{p}$ is a tuple containing all predicates symbols occurring in~$\fh$,
then the formula~$\exists\bf h$ SM$_{\bf p}[\fh \wedge F_{\it graph}]$ has a unique Herbrand model that is also the unique answer set of program~$\mp_c = \tuple{\set{\it in},\fh \wedge F_{\it graph}}$.



==> runningex.tex <==

\section{Running Example: Hamiltonian Cycle}\label{sec:trpr}
\label{sec:motivation}

\begin{comment}
According 
to~\citep{fer05b} and \citep{fer05}, rules of the form~\eqref{eq:ruletraditional} are sufficient 
to capture the meaning of the choice rule construct commonly used in 
answer set programming. For instance, the choice rule ${\tt \{p(X)\}\ar q(X)}$ 
is understood as the rule 
$$p(X)\ar q(X),\ not\ not\ p(X).$$
In this paper we adopt choice rule notation. 
Traditional logic programs cover a substantial practical fragment of the input 
languages used in developing answer set programming applications. %For example, 
%the \hc program from the previous section is a traditional program. 
\end{comment}

Let us consider the \hc problem on a directed graph,
a problem often used to introduce ASP: 
A \hc is a subset of the 
set of edges in a graph that forms a cycle going though each vertex exactly once.
For example, in Figure~\ref{fig:example} we present a sample graph called $G_1$,
where its only Hamiltonian cycle is depicted by edges marked in double lines. Listing~\ref{list:hamiltonian} presents a program in the language of answer set system {\sc clingo}~\citep{geb12}, which encodes the \hc problem.
\begin{figure}
\centering
\begin{tabular}{cc}
%\tiny
\begin{tikzpicture}[scale=0.75, every node/.style={scale=0.75}]
\node[place] (a) {{\it a}};
\node[place] (b)  [right of=a] {{\it b}};
\node[place] (c) [below  of=b] {{\it c}};
\node[place] (d) [below  of=a] {{\it d}};
% (r) edge [loop above] node {} ()
\draw [->,double distance=2pt] (a) to  (b);
\draw [->,double distance=2pt] (b) to  (c);
\draw [->,double distance=2pt] (d) to  (a);
\draw [->,double distance=2pt] (c) to [out=155,in=25] (d);
\draw [->] (d) to [out=-25,in=205] (c);
\end{tikzpicture}
&\hspace{20pt}
\begin{tikzpicture}[shorten >=2pt, auto,scale=0.7, every node/.style={scale=0.7}]
\node[place] (e) {{\it edge}};
\node[place] (v)  [right of=e] {{\it vertex}};
\node[place] (i) [below  of=e] {$\;\;${\it in}$\;\;$ };
\node[place] (r) [below  of=v] {$\;\;\;${\it r}$\;\;$ };
\path[->]
% (r) edge [loop above] node {} ()
(v)   edge[->] node[above] {} (e)
(r)   edge[->] node[above] {} (i)
(i) edge[->] node[below] {} (e)
(r) edge [loop above] node {} ();
\end{tikzpicture}
\end{tabular}
%\normalsize
\caption{Left: graph $G_1$; Right: dependency graph for $\mh^m$.} 
\label{fig:example}
\end{figure}
% \begin{figure}[ht]
\lstinputlisting[
  caption = {Encoding of a Hamiltonian cycle problem using {\sc clingo}. 
%   The program is annotated with \emph{achievements}.
},
  label={list:hamiltonian},
  basicstyle=\ttfamily\small,
  numbers=left,
  stepnumber=2,
]{lp/hamiltonian.tex}
% \end{figure}
% This program is annotated with \emph{achievements}
% following the methodology introduced by~\cite{DBLP:journals/tplp/Lifschitz17}, where he assumes that {\em 
%  ``the programmer would include a comment that states what has been {\em achieved} so far, in a
% certain precise sense.''}
% The properties stated by these achievements are expected to be maintained until the program is
% completed.


To use the program in Listing~\ref{list:hamiltonian} to find Hamiltonian cycles in a graph, one extends it with rules encoding a given graph. For example, rules/facts
in Listing~\ref{list:graph1} specify graph $G_1$.
\lstset{ 
  numbers=none,                    % where to put the line-numbers; possible 
}
\lstinputlisting[
  caption = {Encoding of graph $G_1$ in the language of {\sc clingo}.},
  basicstyle=\ttfamily\small,
  label={list:graph1}
]{lp/graph1.tex}
Each solution/answer set computed by system {\sc clingo} for the program 
in Listing~\ref{list:hamiltonian} extended with a definition of a given graph
corresponds to a Hamiltonian cycle 
%The answer sets of the 
%\hc program above  are in 1-1 correspondence with the Hamiltonian cycles 
of this graph. The {\it in}-atoms occurring in each solution encode these cycles. For instance, 
 the output of {\sc clingo} given lines of code in Listings~\ref{list:hamiltonian} and~\ref{list:graph1}, instructed to find all solutions to the problem, contains the only found solution:\\[5pt]
\lstinline$Answer: 1$\\
\lstinline!in(a,b) in(b,c) in(c,d) in(d,a).!

\vspace{5pt}

We now recite a typical informal reading of some code in Listing~\ref{list:hamiltonian}.
Rules~\mbox{3-4}
state that predicate~$\mathit{r}$ is the transitive closure of the predicate~$\mathit{in}$.
%
Then, rule~5 uses this fact to state that there is no pair of vertices that is not in the transitive closure of~$\mathit{in}$.
%
In other words,
the graph whose vertices are the elements of the relation~$\mathit{vertex}$ and whose edges correspond to the the pairs in the relation~$\mathit{in}$ is strongly connected.
%
As mentioned in the introduction,
one of our goals consists in turning such informal statements into  formal ones.
%
In the paper, we achieve this by grouping rules~\mbox{3-5} into a module and proving that any model of this module satisfies the statement above.

The other thing to note is that, in practice, the presented encoding produces an excessive large ground program.
For this reason rules~3-5 are usually replaced by the rules in Listing~\ref{list:hamiltonian2}~\cite{martru99a}.
% \begin{figure}[ht]
\lstinputlisting[
  caption = {Encoding of a Hamiltonian cycle problem using {\sc clingo}.
%   The program is annotated with \emph{achievements}.
},
  label={list:hamiltonian2},
  basicstyle=\ttfamily\small,
  stepnumber=2,
]{lp/hamiltonian2.tex}
% \end{figure}
If to assume that any input graph  has a vertex named~$a$, then an answer set solver computes identical answers for both of these programs.
This fact is due to the presence of {\tt\#show} directive in line~8.
It states that only  predicate $\mathit{in}/2$
is of interest.
To illustrate the ``equivalence'' between these two programs requires to include the {\tt\#show} directive as the first class citizen in the definition of formal syntax and semantics of a logic program.
To the best of our knowledge this has not been done so far.
The paper introduces the solution to this oversight.

\begin{comment}

{\color{blue} YU: It does not look like we would have enough space for this aspect within IJCAI paper, so it is dropped for now.}

Listing~\ref{list:hamiltonian} provides an intuitive encoding of the \hc problem in ASP. In practice, it is common that lines 12-16 are replaced by the code presented in Listing~\ref{list:hamiltonian2}~\citep{mar99}.
System {\sc clingo} finds the same solution shown in Listing~\ref{list:answer1} for the modified program. 
This modification deserves some comments:
\begin{enumerate}
\item The modified encoding assumes that there is a vertex named ``$a$'' in the input graph.

\item If to remove the $\tt\#show$ directive in both programs, their answer sets will differ. Yet, these answer sets still represent the same \hcs.

\item The achievements in lines 14 and 14b are different. Yet, they allow us to prove the same achievement in line 17.
\end{enumerate}

{
\lstset{ 
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  firstnumber=12
}
\renewcommand*\thelstnumber{\oldstylenums{\the\value{lstnumber}}b}
\lstinputlisting[
  caption = {Alternative encoding of strong connectivity in a Hamiltonian cycle problem.},
  label={list:hamiltonian2}
]{lp/hamiltonian2.tex}
}



\begin{itemize}
    \item {\color{blue} this is probably a place to present the outline of the paper and speak of its main contributions using the motivation example above. The paragraph below would be one of these. } 
\end{itemize}
In Section~\ref{sec:hamiltonian}, we turn achievements into formal statements, prove their correctness,
and show how one can ensure that they are maintained until the program is
completed. These results, for instance, allow us to illustrate
 that if condition~$1$ holds for the considered \hc encoding in  Listing~\ref{list:hamiltonian} then
replacing rules 12-16 by 12b-16b results in an ''\emph{equivalent}'' program.

\end{comment}


% -----------------------------------------------


% Intuitively,
% the facts in Listing~\ref{list:graph1} 
%  define a graph instance by enumerating its edges.
%  The vertices of the graph 
%  are implicit---they are objects that occur in the edge relation\footnote{This 
%  precludes graphs that include isolated vertices, but no graph with isolated vertices can have a Hamiltonian cycle.}.
%  In  Listing~\ref{list:hamiltonian},
% \begin{itemize}
% \setlength\itemsep{0em}
%  \item  we make the  information about the vertices of the graph explicit in Lines 1 and 2  by defining \textit{vertex}-relation that holds over objects that occur in \textit{edge}-relation;
% \item a rule in Line 4 says that any edge may belong to a Hamiltonian cycle;
% \item rules in Lines 6 and 7   impose the restriction that 
% no two edges in a Hamiltonian cycle may start or end at the same vertex;
% \item rules in Lines~9 and 10 define a relation {\it r} 
% (reachable) that is the transitive closure of relation {\it in};
% \item rule in Line 12 imposes the restriction that every vertex in 
% a Hamiltonian cycle 
% must be reachable from every other vertex
% \item Line 14 provides a directive for system {\sc clingo} instructing it to display only atoms with \textit{in} predicates in computed solutions.
% \end{itemize}










==> so.tex <==
\subsection{Second order logic}

We assume a signature~\mbox{$\Sigma=\tuple{\cP,\cC}$}
where~$\cP$ and $\cC$ are (possibly infinite) non-empty sets of \emph{predicate} and \emph{constant} symbols, respectively.
In the remainder of the paper we consider all signatures defined over the same nonempty set of constant symbols so that we may identify a signature with its first component -- its set of predicate symbols~$\cP$.
We also assume two disjoint infinite sets
$\cX$ and $\cH$  of \emph{variables},
where $\cX$ and $\cH$ stand for the sets of first and second order variables, respectively.
We restrict ourselves  to programs without function symbols.
A \emph{term} $t$ is either a constant or a first order variable, i.e., $t \in \cC \cup \cX$.
A \emph{second order (or, SO-formula)}~$\varphi$ is defined by the following grammar:
\[
\varphi \ ::= \ \ \bot 
  \ \ \mid \ \ p(\vec{t}) 
  \ \ \mid \ \ t = t
%   \ \ \mid \ \ \varphi \wedge \varphi 
%   \ \ \mid \ \ \varphi \vee \varphi 
%   \ \ \mid \ \ \varphi \to \varphi
  \ \ \mid \ \ \varphi \otimes \varphi
  \ \ \mid \ \ \exists x \varphi
  \ \ \mid \ \ \forall x \varphi
\]
where $p/n \in \cP \cup \cH$ is a predicate symbol or a second order variable,
$\vec{t}$ is a $n$-tuple of terms,
$t$ is a term,
$\otimes \in \set{\wedge,\vee,\to}$ is a propositional connective
and $x \in \cH \cup \cX$ is a variable.
Formulas $\neg F$ and $\top$ are 
abbreviations for \mbox{$F\to\bot$}
and \mbox{$\bot \to \bot$}, respectively.
A first order formula (or \emph{FO-formula}) is a formula without second order variables.
%
\jcomment{add rules of precedence!}

The set of \emph{free \mbox{FO-variables}} of a term $t$ is the empty set if $t$ is a constant and $\set{t}$ otherwise.
The free \mbox{FO-variables} of $p(\vec{t})$ is the union of the free variables of all elements of $\vec{t}$.
The free \mbox{SO-variables} of $p(\vec{t})$ is either the empty set if $p \in \cP$ or $\set{p}$ if $p \in \cH$.
For boolean formulas, their free FO and \mbox{SO-variables} are the union of the free variables in their subformulas.
The free FO and SO variables in $\exists x \varphi$ and $\forall x \varphi$ are the free FO and SO-variables in $\varphi$, but $x$.
A \emph{sentence} is a formula without free variables.

An interpretation $\cI = \tuple{D,I}$ is a pair where $D$ is a set called the \emph{domain} and $I$ is a function mapping each
constant to an element of $D$
and each predicate symbol $p/n \in \cP$ to a subset of~$D^n$.
We assume that $c^I = c$ for all $c \in D$ and that
$\vec{c}^I = \tuple{c_1^I,\dotsc,c_n^I}$
for any tuple $\vec{c} = \tuple{c_1,\dotsc,c_n}$.
For a set of $n$-tuples $r/n \subseteq D^n$, we assume that $(r/n)^I = (r/n)$.
We will use sets of $n$-tuples, i.e. relations, for defining the semantics of quantifiers over second order variables.
Satisfaction for formulas with respect to an interpretation~$\cI = \tuple{D,I}$ is  defined recursively:
\begin{enumerate}
\item $\cI \not\models \bot$;

% \item $\cI \models p(\vec{c})$ if $\vec{c} \in p$ for any $p \subseteq D^n$ and $\vec{c} \in D^n$

\item $\cI \models p(\vec{c})$ if $\vec{c}^I \in (p/n)^I$ for any $p/n \in \cP \cup \cH$ and $\vec{c} \in (\cC \cup D)^n$

\label{item:p:modelS}
\item $\cI \models t_1=t_2$ if $t_1^I = t_2^I$;

\item $\cI \models \alpha \wedge \beta$ if $\cI \models \alpha$ and $\cI \models \beta$;
\item $\cI \models \alpha \vee \beta$ if $\cI \models \alpha$ or $\cI \models \beta$;
\item $\cI \models \alpha \rightarrow \beta$ if $\cI \not\models \alpha$ or $\cI \models \beta$;
\item $\cI \models \forall x \ \alpha(x)$ if $\cI \models \alpha(c)$ for all $c \in D$ with $x \in \cX$  
\item $\cI \models \exists x \ \alpha(x)$ if $\cI \models \alpha(c)$ for some $c \in D$ with $x \in \cX$

% \item $\cI \models r(\vec{c})$ if $\vec{c}^I \in r$ for any relation $r \subseteq D^n$ and $\vec{c} \in (\cC \cup D)^n$

\item $\cI \models \forall u \ \alpha(u)$ if $\cI \models \alpha(r)$ for all $r \subseteq D^n$ with $u/n \in \cH$
\item ${\cI \models \exists u \alpha(u)}$ if ${\cI \models \alpha(r)}$ for some ${r \subseteq D^n}$\\ with ${u/n \in \cH}$

\end{enumerate}
An interpretation $\cI$ \emph{satisfies} a formula~$\varphi$ iff
\mbox{$\cI \models \varphi$}.
Such interpretations are called {\em models}.
An interpretation is called  {\em Herbrand},  when its domain $D$ coincides with the set $\cC$ of constant symbols.
